Gains-from-Trade in Bilateral Trade with a Broker

We study bilateral trade with a broker, where a buyer and seller interact exclusively through the broker. The broker strategically maximizes her payoff through arbitrage by trading with the buyer and seller at different prices. We study whether the presence of the broker interferes with the mechanism's gains-from-trade (GFT) achieving a constant-factor approximation to the first-best gains-from-trade (FB). We first show that the GFT achieves a $1 / 36$-approximation to the FB even if the broker runs an optimal posted-pricing mechanism under symmetric agents with monotone-hazard-rate distributions. Beyond posted-pricing mechanisms, even if the broker uses an arbitrary incentive-compatible (IC) and individually-rational (IR) mechanism that maximizes her expected profit, we prove that it induces a $1 / 2$-approximation to the first-best GFT when the buyer and seller's distributions are uniform distributions with arbitrary support. This bound is shown to be tight. We complement such results by proving that if the broker uses an arbitrary profit-maximizing IC and IR mechanism, there exists a family of problem instances under which the approximation factor to the first-best GFT becomes arbitrarily bad. We show that this phenomenon persists even if we restrict one of the buyer's or seller's distributions to have a singleton support, or even in the symmetric setting where the buyer and seller have identical distributions.

==> approx-ratio-by-percentiles.tex <==
Let $\mu_F(\alpha)$ denote the $\alpha$-percentile of a cumulative distribution function $F.$ We have the following theorem:

\begin{theorem}
    Suppose $\mu_G(\beta) \le \mu_F(\alpha),$ with $\alpha < 1$ and $\beta > 0.$ Then, if the broker sets $p_s = \mu_G(\beta)$ and $p_b = \mu_F(\alpha),$ $$\textsc{GFT} \ge \beta(1 - \alpha)\textsc{GFT}^*,$$ where $\textsc{GFT}^*$ is the gains-from-trade obtained by any ex-post efficient mechanism.
\end{theorem}
\begin{proof}
    For any $0 \le c \le \mu_G(\beta) \le \mu_F(\alpha),$
\begin{align}
    \int_c^1 (v - c) \, dF(v) &= \int_c^{\mu_F(\alpha)} (v - c) \, dF(v) + \int_{\mu_F(\alpha)}^1 (v - c) \, dF(v) \nonumber\\
    &\le \frac{\alpha}{1 - \alpha}\int_{\mu_F(\alpha)}^1 (v - c) \, dF(v) + \int_{\mu_F(\alpha)}^1 (v - c) \, dF(v) \nonumber\\
    &= \frac{1}{1 - \alpha}\int_{\mu_F(\alpha)}^1 (v - c) \, dF(v),
\end{align}
where we used the fact that $$\int_c^{\mu_F(\alpha)} (v - c) \, dF(v) \le \frac{\alpha}{1 - \alpha}\int_{\mu_F(\alpha)}^1 (v - c) \, dF(v).$$ Observe that this holds because (1) the probability mass of the first integral is at most $\alpha$ while the probability mass of the second integral is exactly $1-\alpha$ and (2) the value of $v - c$ at any point in the probability mass of the second integral is always greater than the value of $v - c$ at any point in the probability mass of the first integral.\ In fact, reusing this idea, we have that
\begin{align}
    \int_{\mu_G(\beta)}^1 \int_c^1 (v - c) \, dF(v) \, dG(c) \le \frac{1 - \beta}{\beta}\int_0^{\mu_G(\beta)} \int_c^1 (v - c) \, dF(v) \, dG(c) \nonumber\\
    \int_0^1 \int_c^1 (v - c) \, dF(v) \, dG(c) \le \frac{1}{\beta}\int_0^{\mu_G(\beta)} \int_c^1 (v - c) \, dF(v) \, dG(c).
\end{align}
Finally, combining inequalities (1) and (2), we obtain $$\int_0^{\mu_G(\beta)} \int_{\mu_F(\alpha)}^1 (v - c) \, dF(v) \, dG(c) \ge \beta(1 - \alpha)\int_0^1 \int_c^1 (v - c) \, dF(v) \, dG(c),$$ as desired.
\end{proof}

==> attempt-posted-pricing.tex <==

% \begin{comment}
---------------BELOW IS AN ATTEMPT FOR POSTED PRICING RESULT---------------

\sscomment{From~\eqref{eq:07021237}, we can further obtain $\FB \le \int_q^p (1-F(x))G(x)dx + \max(G(q),1-F(p))$. Can we get sth from this?}

\sscomment{Below is not actually used as of now. If it will not be used eventually, TODO: remove this or defer to the appendix.}
To analyze the gains-from-trade with such profit-maximizing broker, we first introduce a lemma revealing some structural properties of the optimal prices, which might be useful later.
% \sscomment{Actually this version of the statement can be presented as a corollary of the previous one. Let's have the previous original lemma and present this version as an immediate corollary. (You can check out "History" for the old statements)}
\begin{lemma}
    For regular distributions $F$ and $G$ for which the first-best gains-from-trade is nonzero\footnote{This is a natural assumption because we are only interested in approximating $\FB$ for $F$ and $G$ such that $\FB > 0.$}, any posted-pricing mechanism that maximizes the broker's profit satisfies
    \begin{align*}
        p_b &\ge \phi_G(p_s)\\
        p_s &\le \phi_F(p_b).
    \end{align*}
\end{lemma}
\begin{proof}
    First, note that the broker's optimal profit is strictly greater than zero, since $\FB > 0.$ Now, any posted-pricing mechanism that maximizes the broker's profit satisfies
    \begin{align*}
        (p_b, p_s) &= \argmax_{(p, q) \in [a_1, b_1] \times [a_2, b_2]} (p - q)G(q)(1 - F(p)).
    \end{align*}
    Letting $p = p_b$ and taking the derivative with respect to $q,$ we obtain
    \begin{align*}
        \frac{d}{dq}[(p_b - q)G(q)(1 - F(p_b))] &= (1 - F(p_b))[(p_b - q)g(q) - G(q)].
    \end{align*}    
    Now, assume for the purposes of contradiction that $p_b < \phi_G(p_s).$ Then, noting that $1 - F(p_b) \neq 0$ because the broker's optimal profit is nonzero, we have that
    \begin{itemize}
        \item $(1 - F(p_b))[(p_b - q)g(q) - G(q)] < 0 \Leftrightarrow p_b < \phi_G(q)$
        \item $(1 - F(p_b))[(p_b - q)g(q) - G(q)] = 0 \Leftrightarrow p_b = \phi_G(q)$
        \item $(1 - F(p_b))[(p_b - q)g(q) - G(q)] > 0 \Leftrightarrow p_b > \phi_G(q).$
    \end{itemize}
    Thus, since $\phi_G$ is increasing, we see that $(p_b - q)G(q)(1 - F(p_b))$ increases whenever $p_b > \phi_G(q),$ then remains constant when $p_b = \phi_G(q),$ and finally decreases whenever $p_b < \phi_G(q).$ Then, since $q = p_s$ 
    maximizes $(p_b - q)G(q)(1 - F(p_b))$ by definition and $p_b < \phi_G(q)$ by assumption, we must have that $p_s = a_2.$ But then the optimal profit is $(p_b - a_2)G(a_2)(1 - F(p_b)) = 0,$ a contradiction. Hence,
    \begin{align*}
        p_b \ge \phi_G(p_s).
    \end{align*}

    To prove the second inequality in the lemma, we let $q = p_s$ in the expression for the profit and take the derivative with respect to $p$ to obtain
    \begin{align*}
        \frac{d}{dp}[(p - p_s)G(p_s)(1 - F(p))] &= G(p_S)[-(p - p_s)F'(p) + (1 - F(p))].
    \end{align*}    
    Now, assume for the purposes of contradiction that $p_s > \phi_F(p_b).$ Then, noting that $G(p_s) \neq 0$ because the broker's optimal profit is nonzero, we have that
    \begin{itemize}
        \item $G(p_S)[-(p - p_s)F'(p) + (1 - F(p))] < 0 \Leftrightarrow p_s < \phi_F(p)$
        \item $G(p_S)[-(p - p_s)F'(p) + (1 - F(p))] = 0 \Leftrightarrow p_s = \phi_F(p)$
        \item $G(p_S)[-(p - p_s)F'(p) + (1 - F(p))] > 0 \Leftrightarrow p_s > \phi_F(p).$
    \end{itemize}
    Thus, since $\phi_F$ is increasing, we see that $(p - p_s)G(p_s)(1 - F(p))$ increases whenever $p_s > \phi_F(p),$ then remains constant when $p_s = \phi_F(p),$ and finally decreases whenever $p_s < \phi_F(p).$ Then, since $p = p_b$ 
    maximizes $(p - p_s)G(p_s)(1 - F(p))$ by definition and $p_s > \phi_F(p)$ by assumption, we must have that $p_b = b_1.$ But then the optimal profit is $(b_1 - p_s)G(p_s)(1 - F(b_1)) = 0,$ a contradiction. Hence,
    \begin{align*}
        p_s \le \phi_F(p_b).
    \end{align*}
\end{proof}


\begin{lemma}
    For continuous distributions $F$ and $G$ with overlapping supports $[a_1, b_1]$ and $[a_2, b_2],$ respectively, define $\displaystyle\phi_F(v) = v - \frac{1 - F(v)}{F'(v)}$ and $\displaystyle\phi_G(c) = c + \frac{G(c)}{G'(c)}.$ Then, there exists an optimal mechanism\footnote{We say ``there exists an optimal mechanism'' instead of ``the optimal mechanism'' because there could be multiple maximizing values of $(p, q).$} that satisfies
    \begin{align*}
        p_S(F, G) &= \max\{q \in [a_2, b_2] : p_B(F, G) \ge \phi_G(q)\}\\
        p_B(F, G) &= \max\{p \in [a_1, b_1] : p_S(F, G) \ge \phi_F(p)\}
    \end{align*}
    for any $F$ and $G$ such that $\phi_F$ and $\phi_G$ are increasing.
\end{lemma}
\begin{proof}
    By the definition of the optimal mechanism, 
    \begin{align*}
        (p_B(F, G), p_S(F, G)) &= \argmax_{(p, q) \in [a_1, b_1] \times [a_2, b_2]} (p - q)G(q)(1 - F(p)).
    \end{align*}
    Taking the derivative with respect to $q,$ we obtain
    \begin{align*}
        \frac{\partial}{\partial q}[(p - q)G(q)(1 - F(p))] &= (1 - F(p))[(p - q)G'(q) - G(q)].
    \end{align*}
    Thus, since
    \begin{itemize}
        \item $(p - q)G'(q) - G(q) < 0 \Leftrightarrow p < \phi_G(q)$
        \item $(p - q)G'(q) - G(q) = 0 \Leftrightarrow p = \phi_G(q)$
        \item $(p - q)G'(q) - G(q) > 0 \Leftrightarrow p > \phi_G(q).$
    \end{itemize}
    and since $\phi_G$ is increasing, for $p \in [a_1, b_1],$ we have that $q \in [a_2, b_2]$ maximizes $(p - q)G(q)(1 - F(p))$ if $q$ satisfies $p = \phi_G(q),$ or, if there is no such $q,$ if $q = b_2,$ since $\phi_G$ is continuous. Equivalently, for $p \in [a_1, b_1],$ we have that $q \in [a_2, b_2]$ maximizes $(p - q)G(q)(1 - F(p)),$ if and only if 
    \begin{align*}
        q = \max\{q \in [a_2, b_2] : p \ge \phi_G(q)\}.
    \end{align*}
    In particular, since $q = p_S(F, G)$ maximizes $(p - q)G(q)(1 - F(p))$ for $p = p_B(F, G)$ by definition,
    \begin{align*}
        p_S(F, G) &= \max\{q \in [a_2, b_2] : p_B(F, G) \ge \phi_G(q)\}.
    \end{align*}
    A similar argument will show that 
    \begin{align*}
        p_B(F, G) &= \max\{p \in [a_1, b_1] : p_S(F, G) \ge \phi_F(p)\}.
    \end{align*}
\end{proof}

\subsection{Random Observations}
Assume the support on unit intervals.
Note that
\begin{align}
    \GFT^* = \int_{0}^1 (1-F(x))G(x)dx
\end{align}
In the symmetric case,
\begin{align}
    \GFT(p_B,p_S) 
    &= (1-F(p_B))F(p_S)\parans{\frac{\int_{p_B}^1 vdF(v)}{1-F(p_B)} - \frac{\int_{0}^{p_S}vdF(v)}{F(p_S)}}
    \\
    &\ge
    (1-F(p_B))F(p_S)\parans{p_B - p_S}
    \\
    &= \Pro
\end{align}
\sscomment{(It turns out to be only working for bounded density!) It seems averaging over proper regions for $\Pro$ give constant approximations for bounded distributions, and further MHR distributions. Essentially, let $\alpha_1,\alpha_2,\alpha_3$ be $1/4,2/4,3/4$-quantile. First pick the bigger one between $\int_{0}^{1/2}(1-F(x))F(x)dx$ and $\int_{1/2}^{1}(1-F(x))F(x)dx$. Approximating bigger would imply $1/2$ approximate to the GFT.
Depending on the case above, (1) setting $x= \alpha_3$ and averaging from $y=\alpha_1$ to $y=\alpha_2$ and setting $x= \alpha_2$ and averaging from $y= \alpha=0$ to $\alpha = 1$ or (2) setting $y = \alpha_1$ and averaging from $x = \alpha_2$ to $x = \alpha_3$. or setting $y= \alpha_0$ and averaging from $x= \alpha_1$ to $\alpha_2$.
Essentially, manipulating the inequalities so that the integrand inside $GFT(x,y)$ can be lower bounded by constant times $\int F(x) (1-F(x))dx$ (or for $y$).
For each case of either (1) or (2), summing up the inequalities after properly multiplying it.
Then, we would have sth like $(\frac{\alpha_2 - \alpha_1}{\alpha_3 - \alpha_2} + \frac{\alpha_1 - \alpha_0}{\alpha_2 - \alpha_1} ) GFT \ge \int_{0}^{1/2}F(x) (1-F(x))dx$.
It suffices to properly bound $\Delta \alpha$ from both sides. To this end, we need lemmas on MHR distributions - Lemma 34 from \cite{cai2011extreme} and its variant for the other side inequality, which (I guess) can be shown by setting $G(x) = 1-F(1-x)$ and showing that $G(x)$ is also MHR and applying the same lemma.
Note that if it were to be bounded density distributions rather than MHR, the analysis becomes simpler.}

% This is symmetric case.
% $\alpha_1, \alpha_2,\alpha_3$ be $1/4$, $2/4$, $3/4$, quantile of $F$.
% Let $\alpha_0 = 0 , \alpha_4 = 1$.
% $\GFT \ge \Pro \ge (x-y)(1-F(x))F(y)$, for any $x \ge y \ge 0$.

% $A = \int_{0}^{\alpha_2}F(v) (1-F(v)) dv$
% $B = \int_{\alpha_2}^{1}F(v) (1-F(v)) dv$.
% $A+B = \GFT^*$.
% WLOG, suppose $A \ge B$.
% Approximating $A$ yields $1/$2-apx to the optimal.

% $x = \alpha_3$, averaging over $y = \alpha_0$ to $\alpha_2$.
% $\GFT \ge \frac{1}{\alpha_2 - \alpha_0} \int_{\alpha_0}^{\alpha_2} (\alpha_3 -v ) (1-F(\alpha_3)) F(v) dv$.

% $1-F(\alpha_3) = 1/4$.
% $1-F(v)$ for $v \in [\alpha_0,\alpha_2] = [1/2,1]$.
% Thus, $1-F(\alpha_3) \ge (1-F(v))/4$ for every $v \in [\alpha_0, \alpha_2]$.

% $\alpha_3 - v \ge \alpha_3 - \alpha_2$ for $v \in [\alpha_0,\alpha_2] = [1/2,1]$.

% $RHS \ge \frac{\alpha_3 - \alpha_2}{\alpha_2 - \alpha_0} \int_{\alpha_0}^{\alpha_2} (1-F(v))F(v) dv \ge \frac{\alpha_3 - \alpha_2}{\alpha_2 - \alpha_0}\frac{\GFT^*}{2}$.

% Thus
% $C \cdot \GFT \ge \frac{\alpha_2 - \alpha_0}{\alpha_3-\alpha_2}\GFT \ge \frac{\GFT^*}{2}$.
% Suppose bounded density of $f(v) \in [\delta, \Delta]$.

% Suppose MHR distribution.
% MHR distribution implies regular distribution.
% We can have some inequalities between $\alpha's$, but one side inequality.
% $G(x) = 1-F(1-x)$.
% $g(x) = f(x)$.
% $G(x)$ is also MHR if $F$ is MHR.
% Analogously apply Lemma 36, then there will be other side einequality.
% double side inequality for $\alpha_i,\alpha_j$ , so we can derive some bound here hopefully.





\begin{align}
    \Pro{p_B,p_S} 
    = (p_B - p_S)(1-F(p_B))F(p_S)
    \ge 
    \Pro(m,p_S) 
    = (m - p_S)(1-F(m))F(p_S).
\end{align}

\begin{align*}
    (p_B - p_S) (1-F(p_B)) \ge (m - p_S) /2
\end{align*}

\begin{align*}
    (p_B - p_S) F(p_S) \ge (p_B - m) / 2
\end{align*}

Let $m$ be median of $F$ in the symmetric case. Since $p_B$ and $p_S$ maximizes profit,
\begin{align}
    \Pro(p_B,p_S) \ge (\Pro(m,p_S)+ \Pro(p_B, m))/2,
\end{align}
which implies $F(p_B) - F(p_S) \le 1/2$.
Generally, letting $q_\alpha$ be $\alpha$-quantile of $F$, then we can obtain
\begin{align}
    \alpha F(p_B) - (1-\alpha)F(p_S) \le \alpha^2
\end{align}


Generally, it also follows that
\begin{align}
    \GFT(p_B,p_S) 
    &\ge \Pro + \min(G(p_S),1-F(p_B))\parans{\int_{p_B}^1 (1-F(v))dv + \int_{0}^{p_S}G(c)dc}
    \\
    &\ge
    \Pro + \min(G(p_S),1-F(p_B))\parans{\GFT^* - \int_{p_S}^{p_B}(1-F(x))G(x) dx}
    \\
    &\ge
    (x-y)(1-F(x))F(y) + \min(G(p_S),1-F(p_B))\parans{\GFT^* - \int_{p_S}^{p_B}(1-F(v))F(v) dv}, \explain{in the symmetric case}
    % \\
    % &\ge
    % \min(G(p_S),1/2-F(p_S))\parans{\GFT^* - \int_{p_S}^{p_B}(1-F(x))G(x) dx}
\end{align}
for any $x \ge y \ge 0$.

By taking logarithmic and averaging arguments, one can obtain
\begin{align*}
    \log(\Pro) \ge \frac{1}{2}\Ex{\log(|X-Y|)} - \frac{3}{2},
\end{align*}
which implies that
\begin{align*}
    \Pro \ge \sqrt{e^{-3}e^{\log(|X-Y|)}}.
\end{align*}
% If seller's $1/4$-quantile is smaller than buyer's $1/4$-quantile (which is reasonable assumption), then $\min(G(p_S), 1/2-F(p_S)) \ge 1/4$, so it suffices to bound the final term.



% \sscomment{This looks correct. I tried the case of exponential distribution (symmetric case) which simplifies to $p_B = p_S + 1/\lambda$, and plugging back to maximize the profit, and analyze GFT yields $0.75$ approximation (but probably symmetric exponential allows constant apx for general case as well tho? not sure). Might indeed allow more broader positive results.}
\begin{lemma}
\begin{align*}
    \GFT(p_B, p_S) &= \Pro(p_B, p_S) + F(p_S)\int_{p_B}^1 (1 - F(x)) \, dx + (1 - F(p_B))\int_0^{p_S} F(x) \, dx
\end{align*}
\end{lemma}

\begin{lemma}
    $F(p_B)-F(p_S) \le \min(\int_{p_S}^{p_B}(1-F(t))dt \cdot \ln(\frac{1-F(p_S)}{1-F(p_B)}),\int_{p_S}^{p_B}F(t)dt \cdot \ln(\frac{F(p_B)}{F(p_S)}))$
\end{lemma}

\sscomment{Problematic case for MHR distributions -  when $1-F(p_B) \le F(p_B)$ or $F(p_S) \le 1-F(p_S)$ or $F(p_B) - F(p_S) \ge \max(1-F(p_B), F(p_S))$.}

\sscomment{Discretize the region and }

\begin{lemma}
Let $\displaystyle\GFT([a, b]) = \int_a^b \int_a^v (v - c) \, dF(c) \, dF(v)$ (i.e., the gains-from-trade restricted to $[a, b]$). Then,
\begin{align*}
    \GFT([a, b]) = \int_a^b (F(x) - F(a))(F(b) - F(x)) \, dx.
\end{align*}
\end{lemma}
\begin{lemma}
    Let $F$ be a doubly-regular distribution. Then, for $1 \le m < n < p,$
    \begin{enumerate}[(a)]
        \item $(n - m)(2n - p)(\alpha_p - \alpha_m) \le n(p - m)(\alpha_n - \alpha_m)$
        \item $(m + mn - 2n)(p - n)(\alpha_n - \alpha_m) \le (p + np - 2n)(n - m)(\alpha_p - \alpha_n)$
    \end{enumerate}
\end{lemma}
\begin{proof}
    By the Mean Value Theorem, there exists $a \in (\alpha_m, \alpha_n)$ such that
    \begin{align*}
        F'(a) = \frac{F(\alpha_n) - F(\alpha_m)}{\alpha_n - \alpha_m} = \frac{n - m}{mn(\alpha_n - \alpha_m)},
    \end{align*}
    and there exists $b \in (\alpha_n, \alpha_p)$ such that
    \begin{align*}
        F'(b) = \frac{F(\alpha_p) - F(\alpha_n)}{\alpha_p - \alpha_n} = \frac{p - n}{np(\alpha_p - \alpha_n)}.
    \end{align*}
    Thus, since $F$ is doubly-regular,
    \begin{align*}
        a - \frac{1 - F(a)}{F'(a)} &\le b - \frac{1 - F(b)}{F'(b)}\\
        \alpha_m - \frac{1}{mF'(a)} &\le \alpha_p - \frac{1}{pF'(b)}\\
        \alpha_m - \frac{n}{n - m}(\alpha_n - \alpha_m) &\le \alpha_p - \frac{n}{p - n}(\alpha_p - \alpha_n)\\
        (n - m)(p - n)\alpha_m - n(p - n)(\alpha_n - \alpha_m) &\le (n - m)(p - n)\alpha_p - n(n - m)(\alpha_p - \alpha_n)\\
        (2n - m)(p - n)\alpha_m &\le (n - m)(p - 2n)\alpha_p + n(p - m)\alpha_n\\
        (n - m)(2n - p)(\alpha_p - \alpha_m) &\le n(p - m)(\alpha_n - \alpha_m)
    \end{align*}
    and
    \begin{align*}
        a + \frac{F(a)}{F'(a)} &\le b + \frac{F(b)}{F'(b)}\\
        \alpha_m + \frac{m - 1}{mF'(a)} &\le \alpha_p + \frac{p - 1}{pF'(b)}\\
        \alpha_m + \frac{n(m - 1)}{n - m}(\alpha_n - \alpha_m) &\le \alpha_p + \frac{n(p - 1)}{p - n}(\alpha_p - \alpha_n)\\
        \left(1 - \frac{n(m - 1)}{n - m}\right)\alpha_m + \frac{n(m - 1)}{n - m}\alpha_n &\le \left(1 + \frac{n(p - 1)}{p - n}\right)\alpha_p - \frac{n(p - 1)}{p - n}\alpha_n\\
        (2n - m - mn)(p - n)\alpha_m + n(m - 1)(p - n)\alpha_n &\le (p + np - 2n)(n - m)\alpha_p - n(p - 1)(n - m)\alpha_n\\
        (m + mn - 2n)(p - n)(\alpha_n - \alpha_m) &\le (p + np - 2n)(n - m)(\alpha_p - \alpha_n).
    \end{align*}
\end{proof}
\begin{lemma}
    \gpcomment{incomplete}
    There exists a constant $C$ such that for any optimal posted-price mechanism,
    \begin{align*}
        \GFT^* \le C \cdot \GFT
    \end{align*}
    for any doubly-regular distribution $F,$ where $\GFT = \GFT(p_B, p_S).$
\end{lemma}
\begin{proof}
    We have that
    \begin{align*}
        \GFT^* &= \GFT + \GFT([0, p_B]) + \GFT([p_S, 1]) - \GFT([p_S, p_B])\\
        &= \GFT + \int_0^{p_B} F(x)(F(p_B) - F(x)) \, dx + \int_{p_S}^1 (F(x) - F(p_S))(1 - F(x)) \, dx\\
        &- \int_{p_S}^{p_B} (F(x) - F(p_S))(F(p_B) - F(x)) \, dx\\
        &= \GFT + \left(\int_0^{p_S} F(x)(F(p_B) - F(x)) \, dx + \int_{p_S}^{p_B} F(x)(F(p_B) - F(x)) \, dx\right)\\
        &+ \left(\int_{p_S}^{p_B} (F(x) - F(p_S))(1 - F(x)) \, dx + \int_{p_B}^1 (F(x) - F(p_S))(1 - F(x)) \, dx\right)\\
        &- \int_{p_S}^{p_B} (F(x) - F(p_S))(F(p_B) - F(x)) \, dx\\
        &= \GFT + \int_0^{p_S} F(x)(F(p_B) - F(x)) \, dx + \int_{p_B}^1 (F(x) - F(p_S))(1 - F(x)) \, dx\\
        &+ \int_{p_S}^{p_B} F(x)(F(p_B) - F(x)) \, dx + \int_{p_S}^{p_B} (F(x) - F(p_S))(1 - F(x)) \, dx\\
        &- \int_{p_S}^{p_B} (F(x) - F(p_S))(F(p_B) - F(x)) \, dx\\
        &= \GFT + \int_0^{p_S} F(x)(F(p_B) - F(x)) \, dx + \int_{p_B}^1 (F(x) - F(p_S))(1 - F(x)) \, dx\\
        &+ \int_{p_S}^{p_B} (-F(x)^2 + F(x) - F(p_S) + F(p_B)F(p_S)) \, dx\\
        &= \GFT + \int_0^{p_S} F(x)(F(p_B) - F(x)) \, dx + \int_{p_B}^1 (F(x) - F(p_S))(1 - F(x)) \, dx\\
        &+ \int_{p_S}^{p_B} F(x)(1 - F(x)) \, dx - \Pro(p_B, p_S)\\
        &\le \GFT + F(p_B)\int_0^{p_S} F(x) \, dx + (1 - F(p_S))\int_{p_B}^1 (1 - F(x)) \, dx\\
        &+ (p_B - p_S)F(p_B)(1 - F(p_S)) - \Pro(p_B, p_S)\\
        &\le \GFT + \frac{F(p_B)}{1 - F(p_B)}\GFT +  \frac{1 - F(p_S)}{F(p_S)}\GFT + \frac{1 - F(p_S)}{F(p_S)}\cdot\frac{F(p_B)}{1 - F(p_B)}\Pro(p_B, p_S) - \Pro(p_B, p_S)\\
        &= \GFT + \frac{F(p_B)}{1 - F(p_B)}\GFT +  \frac{1 - F(p_S)}{F(p_S)}\GFT + \frac{F(p_B) - F(p_S)}{F(p_S)(1 - F(p_B))}\Pro(p_B, p_S).
        &\le \GFT + \frac{F(p_B)}{1 - F(p_B)}\GFT +  \frac{1 - F(p_S)}{F(p_S)}\GFT + \frac{F(p_B) - F(p_S)}{F(p_S)(1 - F(p_B))}\GFT\\
        &\le \left(1 + \frac{1}{F(p_S)(1 - F(p_B))}\right)\GFT.
    \end{align*}
\end{proof}
\gpcomment{another proof attempt - unsuccessful}
\begin{proof}
    Since
    \begin{align*}
        \int_0^1 \int_v^1 |v - c| \, dF(c) \, dF(v) &= \int_0^1 \int_0^c |v - c| \, dF(v) \, dF(c) \explain{changing the order of integration}\\
        &= \int_0^1 \int_0^v |c - v| \, dF(c) \, dF(v) \explain{renaming variables}\\
        &= \int_0^1 \int_0^v |v - c| \, dF(c) \, dF(v)\\
        &= \GFT^*,
    \end{align*}
    we have that
    \begin{align*}
        \GFT^* &= \frac{1}{2}\int_0^1 \int_0^1 |v - c| \, dF(c) \, dF(v).
    \end{align*}
    Now, let $\beta_p$ denote the $p$-percentile of $F,$ and let $0 < \epsilon < 1 / 2$ be a quantity to be determined later. Then,
    \begin{align*}
        \GFT^* &= \frac{1}{2}\int_0^1 \int_0^1 |v - c| \, dF(c) \, dF(v)\\
        &= \frac{1}{2}\left(\int_{\beta_{\epsilon}}^{\beta_{1 - \epsilon}} \int_{\beta_{\epsilon}}^{\beta_{1 - \epsilon}} |v - c| \, dF(c) \, dF(v) + \iint_R |v - c| \, dF(c) \, dF(v)\right) \explain{where $R = \{(v, c) : v \not\in [\beta_{\epsilon}, \beta_{1 - \epsilon}] \lor c \not\in [\beta_{\epsilon}, \beta_{1 - \epsilon}]\}$}\\
        &= \frac{1}{2}\left(\int_{\beta_{\epsilon}}^{\beta_{1 - \epsilon}} \int_{\beta_{\epsilon}}^{\beta_{1 - \epsilon}} (\beta_{1 - \epsilon} - \beta_{\epsilon}) \, dF(c) \, dF(v) + \iint_R 1 \, dF(c) \, dF(v)\right)\\
        &\le \frac{1}{2}\left((1 - 2\epsilon)^2(\beta_{1 - \epsilon} - \beta_{\epsilon}) + (1 - (1 - 2\epsilon)^2)\right).
    \end{align*}
    But since
    \begin{align*} 
        (\beta_{1 - \epsilon} - \beta_{\epsilon})\epsilon^2 &\le \Pro\\
        (\beta_{1 - \epsilon} - \beta_{\epsilon}) &\le \frac{\Pro}{\epsilon^2},
    \end{align*}
    we have that
    \begin{align*}
        \GFT^* &\le \frac{1}{2}\left(\frac{(1 - 2\epsilon)^2}{\epsilon^2}\Pro + (1 - (1 - 2\epsilon)^2)\right).
    \end{align*}
    Thus,
    \begin{align*}
        \frac{\GFT^*}{\GFT} &\le \frac{\GFT^*}{\Pro}\\
        &\le \frac{(1 - 2\epsilon)^2\Pro / \epsilon^2 + (1 - (1 - 2\epsilon)^2)}{2\Pro}\\
        &= \frac{(1 - 2\epsilon)^2}{2\epsilon^2} + \frac{(1 - (1 - 2\epsilon)^2)}{2\Pro}.
    \end{align*}
    Now, since $\Pro \le \GFT^* \le 1 / 4,$ taking $\epsilon = \Pro,$ 
    \begin{align*}
    \end{align*}
\end{proof}


\sscomment{Only problematic setting is, Profit is very small, $F(p_B)$ and $F(p_S)$ are both very small, then it suffices to prove that $\GFT^*$ is not that large.}
% \end{comment}

==> inapproximability_bounded.tex <==
\sscomment{If $\phi_F$ is monotone increasing, then it is called regular distribution. A stronger class of distribution is when $(1-F)/f$ itself is monotone decreasing which implies regularity as well. One q: does this counter example show that MHR distribution cannot be a remedy? \Ie, GFT can be arbitrary bad even with MHR distributions?}
\begin{theorem}
    \label{inapprox-thm}
    The gains-from-trade for any incentive-compatible, individually-rational mechanism that maximizes the broker's expected profit can be a $0$-approximation in the worst case.
\end{theorem}
\begin{proof}
    By~\cite{myerson1983efficient}, the gains-from-trade for any incentive-compatible, individually-rational mechanism that maximizes the broker's expected profit is given by 
    \begin{align*}
        \mathsf{GFT} &= \iint (v - c) \mathbf{1}\left\{v - c \ge \frac{1 - F(v)}{F'(v)} + \frac{G(c)}{G'(c)}\right\} \, dF(v) \, dG(c).
    \end{align*}
    Thus, to construct a $F$ and $G$ for which the optimal mechanism achieves a $0$-approximation to the gains-from-trade, it suffices to construct a distribution $F$ such that 
    \begin{align*}
        v = \frac{1 - F(v)}{F'(v)}.
    \end{align*}
    In this way, we always have
    \begin{align*}
        v - c < \frac{1 - F(v)}{F'(v)} + \frac{G(c)}{G'(c)},
    \end{align*}
    so $\GFT = 0.$ Solving the differential equation, we obtain the family of functions 
    \begin{align*}
        F(v) = -\frac{a}{v} + 1
    \end{align*}
    on $[a, \infty).$ However, since~\cite{myerson1983efficient} studied distributions with bounded supports, in the proof below, we truncate $F$ at some point and use linearization to extend the truncated $F$ into a valid CDF.\\\\
    Let $b > a \ge 1,$ and define
    $$F(v) = 
    \begin{cases} 
        -\frac{a}{v} + 1 &\text{if $a \le v \le b$}\\
        \left(-\frac{a}{b} + 1\right) + \frac{a}{b^2}(v - b) &\text{if $b < v \le 2b$}
    \end{cases}.$$
    Note that $F$ is differentiable on $(a, 2b).$ Since $F(a) = 0, F(2b) = 1,$ and $F(v)$ is monotonically increasing, $F$ is a valid CDF. 
    \sscomment{Check the definition of $\phi$. See if it still is regular distribution} Furthermore, 
    \begin{align*}
        \phi_F(v) &= v - \frac{1 - F(v)}{F'(v)}\\
        &= \begin{cases} 
            v - \frac{1 - (-a / v + 1)}{a / v^2} &\text{if $a \le v \le b$}\\
            v - \frac{1 - [(-a / b + 1) + a(v - b) / b^2]}{a / b^2} &\text{if $b < v \le 2b$}
        \end{cases}\\
        &= 0,
    \end{align*}
    so $\phi_F(v)$ is monotonically increasing. Finally, let $G$ be the uniform distribution on $[0, 1].$ Note that $\phi_G(c)$ is also monotonically increasing.
    
    
    We will now show that for any $\epsilon > 0,$ there exists $b$ such that any incentive-compatible, individually-rational mechanism that maximizes the broker's expected profit for the above $F$ and $G$ achieves $\mathsf{GFT} \le \epsilon\mathsf{GFT}^*.$

    By the construction of $F,$ $\displaystyle v - c < \frac{1 - F(v)}{F'(v)} + \frac{G(c)}{G'(c)}$ when $v \in [a, b],$ so
    \begin{align*}
        \GFT &\le \frac{a}{b^2}\int_b^{2b} \int_0^1 (v - c) \, dc \, dv.
    \end{align*}
    In addition,
    \begin{align*}
        \GFT^* &= a\int_a^b \int_0^1 (v - c) \, dc \, \frac{1}{v^2} \, dv + \frac{a}{b^2}\int_b^{2b} \int_0^{1} (v - c) \, dc \, dv.
    \end{align*}
    Thus,
    \begin{align*}
        \frac{\GFT}{\GFT^*} &\le \left(\frac{a}{b^2}\int_b^{2b} \int_0^1 (v - c) \, dc \, dv\right) \bigg / \left(a\int_a^b \int_0^1 (v - c) \, dc \, \frac{1}{v^2} \, dv + \frac{a}{b^2}\int_b^{2b} \int_0^1 (v - c) \, dc \, dv\right)\\
        &= \frac{a(3b - 1)}{2b} \bigg / \left(a\left(\ln\left(\frac{b}{a}\right) + \frac{1}{2b} - \frac{1}{2a}\right) + \frac{a(3b - 1)}{2b}\right),
    \end{align*}
    which approaches $0$ as $b \rightarrow \infty.$ Therefore, the gains-from-trade for any incentive-compatible, individually-rational mechanism that maximizes the broker's expected profit can be arbitrarily inefficient (assuming $\phi_F, \phi_G$ are monotonically increasing).

    \gpcomment{integral calculations below - to be moved to appendix}
    \begin{align*}
        \frac{a}{b^2}\int_b^{2b} \int_0^1 (v - c) \, dc \, dv &= \frac{a}{b^2}\int_b^{2b} \left[vc - \frac{c^2}{2}\right]_0^1 \, dv\\
        &= \frac{a}{b^2}\int_b^{2b} \left(v - \frac{1}{2}\right) \, dv\\
        &= \frac{a}{b^2}\left[\frac{v^2}{2} - \frac{v}{2}\right]_b^{2b}\\
        &= \frac{a}{b^2}\left(\frac{3b^2}{2} - \frac{b}{2}\right)\\
        &= \frac{a(3b - 1)}{2b}
    \end{align*}
    \begin{align*}
        a\int_a^b \int_0^1 (v - c) \, dc \, \frac{1}{v^2} \, dv &= a\int_a^b \left[vc - \frac{c^2}{2}\right]_0^1 \frac{1}{v^2} dv\\
        &= a\int_a^b \left(v - \frac{1}{2}\right)\frac{1}{v^2} \, dv\\
        &= a\left[\ln v + \frac{1}{2v}\right]_a^b\\
        &= a\left(\ln\left(\frac{b}{a}\right) + \frac{1}{2b} - \frac{1}{2a}\right).
    \end{align*}   
\end{proof}

==> known-results.tex <==
\section{Backup}


\paragraph{Questions}
Questions may be as follows.
\begin{enumerate}
    \item Whether the resulting GFT can be a good approximation to the benchmark in hindsight, $\Ex{(v-c) * \Ind{v \ge c}}$. For example, let's start with a simple mechanism for the intermediary.
    \item What happens if the intermediary further randomizes the prices
    \item What mechanisms will further be feasible for him, and which one is the optimal incentive-compatible mechanism and what will be the resulting GFT therein
    \item A naive question though: what if we can reward the intermediary as a lump-sum subsidy from making the trade happen? What should be the lump-sum subsidy to increase GFT?
    \item Further question for more practicality: model digital markets and e-commerce with multiple buyers and multiple sellers. How would the things change?
\end{enumerate}

\sscomment{market matching problem. Stock market.}

\paragraph{Mechanisms}
Several mechanisms that might be of interest.
\begin{enumerate}
    \item Fixed-price mechanism.
        \begin{align*}
            \FP \defeq \sup_{p \in \R} \int_{-\infty}^p \int_{p}^{+\infty} (v-c)dF(v)dG(c).
        \end{align*}
    \item Seller-pricing mechanism.
        \begin{align*}
            \SP \defeq \int_{-\infty}^{+\infty} \int_{p_c}^{+\infty} (v-c)dF(v)dG(c),
        \end{align*}
        where $p_c \in \argmax_p (p-c)(1-F(p))$.
    \item Buyer-pricing mechanism.
        \begin{align*}
            \BP \defeq \int_{-\infty}^{+\infty} \int_{-\infty}^{p_v} (v-c)dG(c)dF(v),
        \end{align*}
        where $p_v \in \argmax_p (v-p)G(p)$.
    \item Random-offerer mechanism.
        \begin{align*}
            \RO \defeq \frac{1}{2}\SP + \frac{1}{2}\BP.
        \end{align*}
\end{enumerate}


\section{Known Results}


\begin{fact}[Folklore]
    It suffices to assume $F$ and $G$ have support on $[0,1]$ with positive densities.
\end{fact}

\begin{fact}[Folklore]
    Buyer-pricing and seller-pricing mechanisms are actually symmetric, thus yielding the same approximation ratio, under some reasonable corresponding assumptions.
\end{fact}

\begin{fact}[\cite{myerson1983efficient}]
    The following holds.
    \begin{align}\label{eq:myerson_identity}
        u_C(1) + u_B(0)
        =
        \int_0^1\int_0^1 \parans{\paranl{v - \frac{1-F(v)}{f(v)}} -  \paranl{c + \frac{G(c)}{g(c)}}} dG(c) dF(v).
    \end{align}
    Furthermore, for any $p$, BIC and IR $x$ exists iff $p(c, \cdot)$ is weakly decreasing over $c$, $p(\cdot, v)$ is weakly increasing over $v$, and
    \begin{align*}
        \int_0^1\int_0^1 \parans{\paranl{v - \frac{1-F(v)}{f(v)}} -  \paranl{c + \frac{G(c)}{g(c)}}} dG(c) dF(v) \ge 0
    \end{align*}
\end{fact}

\begin{fact}[\cite{myerson1983efficient}]
    There is no BIC, IR, WBB, Ex-post efficient mechanism.
\end{fact}

Define $c_S(c,\alpha) = c + \alpha \frac{G(c)}{g(c)}$, and $c_B(v,\alpha) = v - \alpha \frac{1-F(v)}{f(v)}$.
Define $\phi(v) = c_B(v,1)$ and $\psi(c) = c_s(c,1)$.
Let $p^\alpha(c,v) = 1$ if $c_S(c,\alpha) \le c_B(v,\alpha)$ and $0$ otherwise.

\begin{fact}[\cite{myerson1983efficient}]
    If there exists a BIC mechanism such that allocation function $p = p^\alpha$, then it maximizes $\GFT$ among all BIC and IR mechanisms.
    In addition, if both $\phi$ and $\psi$ are increasing functions, then such a mechanism exists.
\end{fact}
For example, if $F$ has MHR and $G$ has MRHR then both $\phi$ and $\psi$ are increasing.

\begin{fact}[\cite{blumrosen2016approximating}]
    Lower bound for approximation ratio is $e/2\approx 1.359$.
    This even holds when both $F$ and $G$ have MHR.
\end{fact}
This lower bound stems from the Myerson and Satterthwaite's characterization on the optimal \GFT.
Formally, consider regular $\phi$ and $\psi$, \ie both are increasing.
Then, a mechanism $(x,p)$ such that $p = p^\alpha$ exists which maximizes $\GFT$.
One can compute $\alpha$ from \eqref{eq:myerson_identity} using $\LHS = 0$.


\begin{fact}[\cite{blumrosen2016approximating}]
    If $F$ has MHR with concave hazard rate, then $(e/2) \SP \ge \FB$.
\end{fact}

\begin{fact}[\cite{fei2022improved}]
    Upper bound for approximation ratio is $\approx 3.15$-approximation, by \RO.
\end{fact}

\begin{fact}[\cite{fei2022improved}]
    If $F$ has MHR, then $(e-1) \SP \ge \FB$, and this is tight.
\end{fact}
Worst-case instance is when $G$ is a point mass on $0$, and $F$ is $1-e^{-x}$ for $x \le 1-\delta$, and then quadratic for $1-\delta < x \le 1$.
Upper bound is from the following useful observations.
\begin{observation}
    \begin{align*}
        \FB(c) 
        = 
        \int_{c}^1 (1-F(v)) dv 
        = 
        \int_{c}^{\phi^{-1}(c)} (1-F(v)) dv
        +
        \int_{\phi^{-1}(c)}^{1} (1-F(v)) dv
    \end{align*}
\end{observation}


\begin{fact}[\cite{fei2022improved}]
    As a corollary of the above facts, if $G$ has MRHR, then $(e-1)\BP \ge \FB$, and this is tight. In addition, $1/(e-1)\FB \le \RO \le (1-1/e)\FB$.
\end{fact}

\begin{fact}[Tamuz]
    \begin{align*}
        \sup_p p (1-F(p)) \ge \frac{1}{e}\exp(\Ex{\ln X}),
    \end{align*}
    where the equality holds when $F$ satisfies $F(v) = 1-u/v$ for $v > u$ and otherwise $0$ where $u = \sup_p p (1-F(p))t$.
\end{fact}

Decomposition Lemma in Bilateral Trade: A Regret Minimization Perspective.



==> model.tex <==



\section{Problem Setup}
In a bilateral trade problem, there is a seller with an item who tries to sell it to a buyer.
Both the buyer's and seller's values are private, and are independently drawn from cumulative distributions (CDF) $F$ and $G$, respectively.
We write $v$ and $c$ to denote the buyer's and seller's values.
% We assume that $v$ and $c$ are independent.
If a trade occurs between the seller and buyer with $c$ and $v$, the society realizes the increment of the welfare of amount $v-c$.
We are interested in designing a mechanism which decides the allocation function (probability) $x(\tilde{v},\tilde{c})$ given the reported values.
Then, the \emph{gains-from-trade}\footnote{Note that this differs from the social welfare since social welfare is $v$ even if the trade does not occur.} (GFT) is defined by the expected amount of increased utility from trade, \ie
\begin{align*}
    \GFT = \Exu{v \sim F, c \sim G}{(v-c)\cdot x(v,c)}.
\end{align*}
If there exists an omniscient social planner who can observe the private values and governs the trade, it can enforce the trade to occur whenever the buyer's value is larger than the seller's one.
Such an ideal mechanism induces $x(v,c) = \Ind{v \ge c}$, and the resulting optimal $\GFT$ is defined as the \emph{first-best} GFT, \ie 
\begin{align*}
    \FB =  \Exu{v \sim F, c \sim G}{(v-c) \Ind{v \ge c}}.
\end{align*}
A mechanism is defined to be \emph{ex-post efficient} if it achieves the first-best GFT.
In fact, however, the seminal result by~\cite{myerson1983efficient} asserts that it is not possible to construct a mechanism that is simultaneously (i) Bayesian incentive-compatible (BIC), (ii) individually rational\footnote{A mechanism is IR if all the participants are not worse off by not joining the game.} (IR),(iii) weakly budget balanced\footnote{A mechanism is WBB if the payment from the buyer is always at least the payment to the seller in an ex-post manner.} (WBB), and (iv) ex-post efficient.

\paragraph{Bilateral Trade with Broker}
In our setup, there exists a broker who governs the entire trade, and thus the buyer and seller can only exclusively interact through the broker.
However, the broker is not interested in maximizing GFT, but tries to maximize its own profit by constituting an arbitrage by buying from the seller at lower price and selling to the buyer at higher price.
Following~\cite{myerson1983efficient}, we assume that the broker can be a net source or sink of monetary transfer in the game, but cannot own the item by itself.
Alternatively, the broker realizes the value $0$ for the item.

Essentially, the broker's mechanism $\Mec = (x,p)$ is defined by an allocation function $x: \R_{\ge 0}^2 \to [0,1]$ that maps the reported values to a probability that the item is transferred from the seller to buyer, and a payment function $q: \R_{\ge 0}^2 \to \R_{\ge 0}^2$ that maps the reported values to the payment $p = (q_s,p_b)$ with $q_s$ being the expected payment from the broker to the seller, and $q_b$ the one from the buyer to broker.\footnote{Note here that it is defined to be expected payment, as the mechanism might randomize the payment as well.}
Remark here that both $q_b$ and $q_s$ are defined to be nonnegative prices although the direction of the monetary transfer is opposite.
Note here that the broker's net profit can be defined as 
\begin{align*}
    \Pro = \int_{0}^{\infty}\int_{0}^{\infty}\parans{q_b(v,c) - q_s(v,c)} dF(v) dG(c)
\end{align*}
Correspondingly, the buyer's expected utility from reporting $\tilde{v}$ can be written as $u_b(\tilde{v},c) = x(\tilde{v},c) \cdot v - q_b(\tilde{v},c)$, and similarly the seller's expected utility from reporting $\tilde{c}$ is $u_s(v, \tilde{c}) = q_s(v, \tilde{c}) - x(v,\tilde{c}) \cdot c$, assuming truthful reporting of the others.

A broker's mechanism is \emph{Bayes incentive-compatible} (BIC) if it satisfies 
\begin{align*}
    \Exu{c \sim G}{u_b(v,c)} &\ge \Exu{c \sim G}{u_b(\tilde{v},c)}\\
    \Exu{v \sim F}{u_s(v,c)} &\ge \Exu{v \sim F}{u_s(v,\tilde{c})},
\end{align*}
given that the true private values are realized to be $v$ and $c$, respectively.
The first inequality denotes the buyer's ex-interim incentive to truthfully report the private value, and the second one corresponds to the seller's one.

Analogously, a broker's mechanism is \emph{dominant-strategy incentive-compatible} (DSIC) if it satisfies
\begin{align*}
    u_b(v,c) &\ge u_b(\tilde{v},c)
    \\
    u_s(v,c) &\ge u_s(v,\tilde{c}),
\end{align*}
for every $v$ and $c$.

\section{Posted Pricing Mechanism}
Consider a broker who implements a posted pricing mechanism.
Posted pricing is widely adopted in many real world applications \sscomment{give some examples} due to its simplicity and transparency.
\sscomment{Provide an example that the broker deviates from the announced rule and increases profit. $0.2$ and $0.8$ is reported from seller and buyer respectively, but the broker announces as if it were $0.25$ and $0.75$. Then, original profit is $0.7 - 0.3 = 0.4$ whereas the new profit is $0.75 - 0.25 = 0.5$. Can we argue this formally? The only credible DSIC mechanism is posted pricing?}
In addition, in the standard setting without broker, it is shown to be the only mechanism that satisfies budget balancedness and DSIC by \sscomment{CITE}.

Precisely, a posted pricing mechanism consists of two fixed prices $p = (p_b,p_s)$ such that the broker offers the buyer to buy at price $p_b$ and the seller to sell at $p_s$.
Since the broker strategizes to maximize its profit, it should follow that $p_b \ge p_s$ as the broker does not want to run a deficit.
Then, the buyer and the seller decides whether to accept the offers in a \emph{take-it-or-leave} manner.
Once both the players decide to take the offer, the trade occurs and the item is transferred from the seller to the buyer.

Under the posted pricing mechanism with $p = (p_b,p_s)$, the broker's profit can be simplified as
\begin{align*}
    \Pro = \int_{0}^{p_s}\int_{p_b}^{\infty} (p_b-p_s) dF(v) dG(c).
\end{align*}

\subsection{Constant approximation with regular distributions}
\sscomment{This section should be adjusted w.r.t. our result. Leave it empty for now.}
Our first result states that the resulting GFT is a constant approximation to the first-best GFT if the buyer and the seller's distributions are identical and satisfy a regularity.

Formally, the buyer's distribution is regular if $\phi_F(x) = x - \frac{1-F(x)}{f(x)}$ is nondecreasing for $x$ where $f(x)$ is probability density function (pdf) of $F$.
Analogously, the seller's distribution is regular if $\phi_G(x) = x + \frac{G(x)}{g(x)}$ is nondecreasing for $x$ where $g(x)$ is p.d.f. of $G$.




\paragraph{Quantile based pricing}




\input{approx-ratio-by-percentiles}


\sscomment{prove that Fixed pricing is the only DSIC and WBB for bilateral trade with broker? at least this is true for without broker (but here SBB and DSIC and fixed price), see Robust trading mechanisms.}




==> optimal-posted-price.tex <==
\begin{definition}
    A \textit{posted-price mechanism} $M = (p_B(\cdot, \cdot), p_S(\cdot, \cdot))$ is a mechanism in which the broker simultaneously offers to buy the item from the seller at a price of $p_S(F, G)$ and sell the item to the buyer at a price of $p_B(F, G).$ where $F$ and $G$ are the distributions of the buyer's and seller's valuations, respectively. The buyer and seller then report their respective valuations $v \sim F$ and $c \sim G$ to the broker. A trade occurs if and only if both $v \ge p_B(F, G)$ and $c \le p_S(F, G),$ upon which the seller receives $p_S(F, G)$ and the buyer pays $p_B(F, G).$
\end{definition}
Note that posted-price mechanisms are dominant-strategy incentive-compatible and individually-rational. In addition, for ease of exposition, we will restrict $F$ and $G$ to continuous distributions with bounded (nonnegative) supports $[a_1, b_1]$ and $[a_2, b_2],$ respectively.\\\\
From the above definition, it is clear that the posted-price mechanism that maximizes the expected profit for the broker is given by 
\begin{align*}
    (p_B(F, G), p_S(F, G)) &= \argmax_{(p, q) \in [a_1, b_1] \times [a_2, b_2]} \int_p^{b_1} \int_{a_2}^q (p - q) \, dG(c) \, dF(v)\\
    &= \argmax_{(p, q) \in [a_1, b_1] \times [a_2, b_2]} (p - q)G(q)(1 - F(p)).
\end{align*}
We seek to analyze the gains-from-trade of this optimal mechanism compared to the gains-from-trade of an ex-post efficient mechanism. 
\begin{lemma}
    For continuous distributions $F$ and $G$ with overlapping supports $[a_1, b_1]$ and $[a_2, b_2],$ respectively, define $\displaystyle\phi_F(v) = v - \frac{1 - F(v)}{F'(v)}$ and $\displaystyle\phi_G(c) = c + \frac{G(c)}{G'(c)}.$ Then, there exists an optimal mechanism\footnote{We say ``there exists an optimal mechanism'' instead of ``the optimal mechanism'' because there could be multiple maximizing values of $(p, q).$} that satisfies
    \begin{align*}
        p_S(F, G) &= \max\{q \in [a_2, b_2] : p_B(F, G) \ge \phi_G(q)\}\\
        p_B(F, G) &= \max\{p \in [a_1, b_1] : p_S(F, G) \ge \phi_F(p)\}
    \end{align*}
    for any $F$ and $G$ such that $\phi_F$ and $\phi_G$ are increasing.
\end{lemma}
\begin{proof}
    By the definition of the optimal mechanism, 
    \begin{align*}
        (p_B(F, G), p_S(F, G)) &= \argmax_{(p, q) \in [a_1, b_1] \times [a_2, b_2]} (p - q)G(q)(1 - F(p)).
    \end{align*}
    Taking the derivative with respect to $q,$ we obtain
    \begin{align*}
        \frac{\partial}{\partial q}[(p - q)G(q)(1 - F(p))] &= (1 - F(p))[(p - q)G'(q) - G(q)].
    \end{align*}
    Thus, since
    \begin{itemize}
        \item $(p - q)G'(q) - G(q) < 0 \Leftrightarrow p < \phi_G(q)$
        \item $(p - q)G'(q) - G(q) = 0 \Leftrightarrow p = \phi_G(q)$
        \item $(p - q)G'(q) - G(q) > 0 \Leftrightarrow p > \phi_G(q).$
    \end{itemize}
    and since $\phi_G$ is increasing, for $p \in [a_1, b_1],$ we have that $q \in [a_2, b_2]$ maximizes $(p - q)G(q)(1 - F(p))$ if $q$ satisfies $p = \phi_G(q),$ or, if there is no such $q,$ if $q = b_2,$ since $\phi_G$ is continuous. Equivalently, for $p \in [a_1, b_1],$ we have that $q \in [a_2, b_2]$ maximizes $(p - q)G(q)(1 - F(p)),$ if and only if 
    \begin{align*}
        q = \max\{q \in [a_2, b_2] : p \ge \phi_G(q)\}.
    \end{align*}
    In particular, since $q = p_S(F, G)$ maximizes $(p - q)G(q)(1 - F(p))$ for $p = p_B(F, G)$ by definition,
    \begin{align*}
        p_S(F, G) &= \max\{q \in [a_2, b_2] : p_B(F, G) \ge \phi_G(q)\}.
    \end{align*}
    A similar argument will show that 
    \begin{align*}
        p_B(F, G) &= \max\{p \in [a_1, b_1] : p_S(F, G) \ge \phi_F(p)\}.
    \end{align*}
\end{proof}

\subsection{Random Observations}
Assume the support on unit intervals.
Note that
\begin{align}
    \GFT^* = \int_{0}^1 (1-F(x))G(x)dx
\end{align}
In the symmetric case,
\begin{align}
    \GFT(p_B,p_S) 
    &= (1-F(p_B))F(p_S)\parans{\frac{\int_{p_B}^1 vdF(v)}{1-F(p_B)} - \frac{\int_{0}^{p_S}vdF(v)}{F(p_S)}}
    \\
    &\ge
    (1-F(p_B))F(p_S)\parans{p_B - p_S}
    \\
    &= \Pro
\end{align}
\sscomment{(It turns out to be only working for bounded density!) It seems averaging over proper regions for $\Pro$ give constant approximations for bounded distributions, and further MHR distributions. Essentially, let $\alpha_1,\alpha_2,\alpha_3$ be $1/4,2/4,3/4$-quantile. First pick the bigger one between $\int_{0}^{1/2}(1-F(x))F(x)dx$ and $\int_{1/2}^{1}(1-F(x))F(x)dx$. Approximating bigger would imply $1/2$ approximate to the GFT.
Depending on the case above, (1) setting $x= \alpha_3$ and averaging from $y=\alpha_1$ to $y=\alpha_2$ and setting $x= \alpha_2$ and averaging from $y= \alpha=0$ to $\alpha = 1$ or (2) setting $y = \alpha_1$ and averaging from $x = \alpha_2$ to $x = \alpha_3$. or setting $y= \alpha_0$ and averaging from $x= \alpha_1$ to $\alpha_2$.
Essentially, manipulating the inequalities so that the integrand inside $GFT(x,y)$ can be lower bounded by constant times $\int F(x) (1-F(x))dx$ (or for $y$).
For each case of either (1) or (2), summing up the inequalities after properly multiplying it.
Then, we would have sth like $(\frac{\alpha_2 - \alpha_1}{\alpha_3 - \alpha_2} + \frac{\alpha_1 - \alpha_0}{\alpha_2 - \alpha_1} ) GFT \ge \int_{0}^{1/2}F(x) (1-F(x))dx$.
It suffices to properly bound $\Delta \alpha$ from both sides. To this end, we need lemmas on MHR distributions - Lemma 34 from \cite{cai2011extreme} and its variant for the other side inequality, which (I guess) can be shown by setting $G(x) = 1-F(1-x)$ and showing that $G(x)$ is also MHR and applying the same lemma.
Note that if it were to be bounded density distributions rather than MHR, the analysis becomes simpler.}

% This is symmetric case.
% $\alpha_1, \alpha_2,\alpha_3$ be $1/4$, $2/4$, $3/4$, quantile of $F$.
% Let $\alpha_0 = 0 , \alpha_4 = 1$.
% $\GFT \ge \Pro \ge (x-y)(1-F(x))F(y)$, for any $x \ge y \ge 0$.

% $A = \int_{0}^{\alpha_2}F(v) (1-F(v)) dv$
% $B = \int_{\alpha_2}^{1}F(v) (1-F(v)) dv$.
% $A+B = \GFT^*$.
% WLOG, suppose $A \ge B$.
% Approximating $A$ yields $1/$2-apx to the optimal.

% $x = \alpha_3$, averaging over $y = \alpha_0$ to $\alpha_2$.
% $\GFT \ge \frac{1}{\alpha_2 - \alpha_0} \int_{\alpha_0}^{\alpha_2} (\alpha_3 -v ) (1-F(\alpha_3)) F(v) dv$.

% $1-F(\alpha_3) = 1/4$.
% $1-F(v)$ for $v \in [\alpha_0,\alpha_2] = [1/2,1]$.
% Thus, $1-F(\alpha_3) \ge (1-F(v))/4$ for every $v \in [\alpha_0, \alpha_2]$.

% $\alpha_3 - v \ge \alpha_3 - \alpha_2$ for $v \in [\alpha_0,\alpha_2] = [1/2,1]$.

% $RHS \ge \frac{\alpha_3 - \alpha_2}{\alpha_2 - \alpha_0} \int_{\alpha_0}^{\alpha_2} (1-F(v))F(v) dv \ge \frac{\alpha_3 - \alpha_2}{\alpha_2 - \alpha_0}\frac{\GFT^*}{2}$.

% Thus
% $C \cdot \GFT \ge \frac{\alpha_2 - \alpha_0}{\alpha_3-\alpha_2}\GFT \ge \frac{\GFT^*}{2}$.
% Suppose bounded density of $f(v) \in [\delta, \Delta]$.

% Suppose MHR distribution.
% MHR distribution implies regular distribution.
% We can have some inequalities between $\alpha's$, but one side inequality.
% $G(x) = 1-F(1-x)$.
% $g(x) = f(x)$.
% $G(x)$ is also MHR if $F$ is MHR.
% Analogously apply Lemma 36, then there will be other side einequality.
% double side inequality for $\alpha_i,\alpha_j$ , so we can derive some bound here hopefully.





\begin{align}
    \Pro{p_B,p_S} 
    = (p_B - p_S)(1-F(p_B))F(p_S)
    \ge 
    \Pro(m,p_S) 
    = (m - p_S)(1-F(m))F(p_S).
\end{align}

\begin{align*}
    (p_B - p_S) (1-F(p_B)) \ge (m - p_S) /2
\end{align*}

\begin{align*}
    (p_B - p_S) F(p_S) \ge (p_B - m) / 2
\end{align*}

Let $m$ be median of $F$ in the symmetric case. Since $p_B$ and $p_S$ maximizes profit,
\begin{align}
    \Pro(p_B,p_S) \ge (\Pro(m,p_S)+ \Pro(p_B, m))/2,
\end{align}
which implies $F(p_B) - F(p_S) \le 1/2$.
Generally, letting $q_\alpha$ be $\alpha$-quantile of $F$, then we can obtain
\begin{align}
    \alpha F(p_B) - (1-\alpha)F(p_S) \le \alpha^2
\end{align}


Generally, it also follows that
\begin{align}
    \GFT(p_B,p_S) 
    &\ge \Pro + \min(G(p_S),1-F(p_B))\parans{\int_{p_B}^1 (1-F(v))dv + \int_{0}^{p_S}G(c)dc}
    \\
    &\ge
    \Pro + \min(G(p_S),1-F(p_B))\parans{\GFT^* - \int_{p_S}^{p_B}(1-F(x))G(x) dx}
    \\
    &\ge
    (x-y)(1-F(x))F(y) + \min(G(p_S),1-F(p_B))\parans{\GFT^* - \int_{p_S}^{p_B}(1-F(v))F(v) dv}, \explain{in the symmetric case}
    % \\
    % &\ge
    % \min(G(p_S),1/2-F(p_S))\parans{\GFT^* - \int_{p_S}^{p_B}(1-F(x))G(x) dx}
\end{align}
for any $x \ge y \ge 0$.

By taking logarithmic and averaging arguments, one can obtain
\begin{align*}
    \log(\Pro) \ge \frac{1}{2}\Ex{\log(|X-Y|)} - \frac{3}{2},
\end{align*}
which implies that
\begin{align*}
    \Pro \ge \sqrt{e^{-3}e^{\log(|X-Y|)}}.
\end{align*}
% If seller's $1/4$-quantile is smaller than buyer's $1/4$-quantile (which is reasonable assumption), then $\min(G(p_S), 1/2-F(p_S)) \ge 1/4$, so it suffices to bound the final term.



% \sscomment{This looks correct. I tried the case of exponential distribution (symmetric case) which simplifies to $p_B = p_S + 1/\lambda$, and plugging back to maximize the profit, and analyze GFT yields $0.75$ approximation (but probably symmetric exponential allows constant apx for general case as well tho? not sure). Might indeed allow more broader positive results.}
\begin{lemma}
\begin{align*}
    \GFT(p_B, p_S) &= \Pro(p_B, p_S) + F(p_S)\int_{p_B}^1 (1 - F(x)) \, dx + (1 - F(p_B))\int_0^{p_S} F(x) \, dx
\end{align*}
\end{lemma}
\begin{lemma}
Let $\displaystyle\GFT([a, b]) = \int_a^b \int_a^v (v - c) \, dF(c) \, dF(v)$ (i.e., the gains-from-trade restricted to $[a, b]$). Then,
\begin{align*}
    \GFT([a, b]) = \int_a^b (F(x) - F(a))(F(b) - F(x)) \, dx.
\end{align*}
\end{lemma}
\begin{lemma}
    Let $F$ be a doubly-regular distribution. Then, for $1 \le m < n < p,$
    \begin{enumerate}[(a)]
        \item $(n - m)(2n - p)(\alpha_p - \alpha_m) \le n(p - m)(\alpha_n - \alpha_m)$
        \item $(m + mn - 2n)(p - n)(\alpha_n - \alpha_m) \le (p + np - 2n)(n - m)(\alpha_p - \alpha_n)$
    \end{enumerate}
\end{lemma}
\begin{proof}
    By the Mean Value Theorem, there exists $a \in (\alpha_m, \alpha_n)$ such that
    \begin{align*}
        F'(a) = \frac{F(\alpha_n) - F(\alpha_m)}{\alpha_n - \alpha_m} = \frac{n - m}{mn(\alpha_n - \alpha_m)},
    \end{align*}
    and there exists $b \in (\alpha_n, \alpha_p)$ such that
    \begin{align*}
        F'(b) = \frac{F(\alpha_p) - F(\alpha_n)}{\alpha_p - \alpha_n} = \frac{p - n}{np(\alpha_p - \alpha_n)}.
    \end{align*}
    Thus, since $F$ is doubly-regular,
    \begin{align*}
        a - \frac{1 - F(a)}{F'(a)} &\le b - \frac{1 - F(b)}{F'(b)}\\
        \alpha_m - \frac{1}{mF'(a)} &\le \alpha_p - \frac{1}{pF'(b)}\\
        \alpha_m - \frac{n}{n - m}(\alpha_n - \alpha_m) &\le \alpha_p - \frac{n}{p - n}(\alpha_p - \alpha_n)\\
        (n - m)(p - n)\alpha_m - n(p - n)(\alpha_n - \alpha_m) &\le (n - m)(p - n)\alpha_p - n(n - m)(\alpha_p - \alpha_n)\\
        (2n - m)(p - n)\alpha_m &\le (n - m)(p - 2n)\alpha_p + n(p - m)\alpha_n\\
        (n - m)(2n - p)(\alpha_p - \alpha_m) &\le n(p - m)(\alpha_n - \alpha_m)
    \end{align*}
    and
    \begin{align*}
        a + \frac{F(a)}{F'(a)} &\le b + \frac{F(b)}{F'(b)}\\
        \alpha_m + \frac{m - 1}{mF'(a)} &\le \alpha_p + \frac{p - 1}{pF'(b)}\\
        \alpha_m + \frac{n(m - 1)}{n - m}(\alpha_n - \alpha_m) &\le \alpha_p + \frac{n(p - 1)}{p - n}(\alpha_p - \alpha_n)\\
        \left(1 - \frac{n(m - 1)}{n - m}\right)\alpha_m + \frac{n(m - 1)}{n - m}\alpha_n &\le \left(1 + \frac{n(p - 1)}{p - n}\right)\alpha_p - \frac{n(p - 1)}{p - n}\alpha_n\\
        (2n - m - mn)(p - n)\alpha_m + n(m - 1)(p - n)\alpha_n &\le (p + np - 2n)(n - m)\alpha_p - n(p - 1)(n - m)\alpha_n\\
        (m + mn - 2n)(p - n)(\alpha_n - \alpha_m) &\le (p + np - 2n)(n - m)(\alpha_p - \alpha_n).
    \end{align*}
\end{proof}
\begin{lemma}
    \gpcomment{incomplete}
    There exists a constant $C$ such that for any optimal posted-price mechanism,
    \begin{align*}
        \GFT^* \le C \cdot \GFT
    \end{align*}
    for any doubly-regular distribution $F,$ where $\GFT = \GFT(p_B, p_S).$
\end{lemma}
\begin{proof}
    We have that
    \begin{align*}
        \GFT^* &= \GFT + \GFT([0, p_B]) + \GFT([p_S, 1]) - \GFT([p_S, p_B])\\
        &= \GFT + \int_0^{p_B} F(x)(F(p_B) - F(x)) \, dx + \int_{p_S}^1 (F(x) - F(p_S))(1 - F(x)) \, dx\\
        &- \int_{p_S}^{p_B} (F(x) - F(p_S))(F(p_B) - F(x)) \, dx\\
        &= \GFT + \left(\int_0^{p_S} F(x)(F(p_B) - F(x)) \, dx + \int_{p_S}^{p_B} F(x)(F(p_B) - F(x)) \, dx\right)\\
        &+ \left(\int_{p_S}^{p_B} (F(x) - F(p_S))(1 - F(x)) \, dx + \int_{p_B}^1 (F(x) - F(p_S))(1 - F(x)) \, dx\right)\\
        &- \int_{p_S}^{p_B} (F(x) - F(p_S))(F(p_B) - F(x)) \, dx\\
        &= \GFT + \int_0^{p_S} F(x)(F(p_B) - F(x)) \, dx + \int_{p_B}^1 (F(x) - F(p_S))(1 - F(x)) \, dx\\
        &+ \int_{p_S}^{p_B} F(x)(F(p_B) - F(x)) \, dx + \int_{p_S}^{p_B} (F(x) - F(p_S))(1 - F(x)) \, dx\\
        &- \int_{p_S}^{p_B} (F(x) - F(p_S))(F(p_B) - F(x)) \, dx\\
        &= \GFT + \int_0^{p_S} F(x)(F(p_B) - F(x)) \, dx + \int_{p_B}^1 (F(x) - F(p_S))(1 - F(x)) \, dx\\
        &+ \int_{p_S}^{p_B} (-F(x)^2 + F(x) - F(p_S) + F(p_B)F(p_S)) \, dx\\
        &= \GFT + \int_0^{p_S} F(x)(F(p_B) - F(x)) \, dx + \int_{p_B}^1 (F(x) - F(p_S))(1 - F(x)) \, dx\\
        &+ \int_{p_S}^{p_B} F(x)(1 - F(x)) \, dx - \Pro(p_B, p_S)\\
        &\le \GFT + F(p_B)\int_0^{p_S} F(x) \, dx + (1 - F(p_S))\int_{p_B}^1 (1 - F(x)) \, dx\\
        &+ (p_B - p_S)F(p_B)(1 - F(p_S)) - \Pro(p_B, p_S)\\
        &\le \GFT + \frac{F(p_B)}{1 - F(p_B)}\GFT +  \frac{1 - F(p_S)}{F(p_S)}\GFT + \frac{1 - F(p_S)}{F(p_S)}\cdot\frac{F(p_B)}{1 - F(p_B)}\Pro(p_B, p_S) - \Pro(p_B, p_S)\\
        &= \GFT + \frac{F(p_B)}{1 - F(p_B)}\GFT +  \frac{1 - F(p_S)}{F(p_S)}\GFT + \frac{F(p_B) - F(p_S)}{F(p_S)(1 - F(p_B))}\Pro(p_B, p_S).
        &\le \GFT + \frac{F(p_B)}{1 - F(p_B)}\GFT +  \frac{1 - F(p_S)}{F(p_S)}\GFT + \frac{F(p_B) - F(p_S)}{F(p_S)(1 - F(p_B))}\GFT\\
        &\le \left(1 + \frac{1}{F(p_S)(1 - F(p_B))}\right)\GFT.
    \end{align*}
\end{proof}
\gpcomment{another proof attempt - unsuccessful}
\begin{proof}
    Since
    \begin{align*}
        \int_0^1 \int_v^1 |v - c| \, dF(c) \, dF(v) &= \int_0^1 \int_0^c |v - c| \, dF(v) \, dF(c) \explain{changing the order of integration}\\
        &= \int_0^1 \int_0^v |c - v| \, dF(c) \, dF(v) \explain{renaming variables}\\
        &= \int_0^1 \int_0^v |v - c| \, dF(c) \, dF(v)\\
        &= \GFT^*,
    \end{align*}
    we have that
    \begin{align*}
        \GFT^* &= \frac{1}{2}\int_0^1 \int_0^1 |v - c| \, dF(c) \, dF(v).
    \end{align*}
    Now, let $\beta_p$ denote the $p$-percentile of $F,$ and let $0 < \epsilon < 1 / 2$ be a quantity to be determined later. Then,
    \begin{align*}
        \GFT^* &= \frac{1}{2}\int_0^1 \int_0^1 |v - c| \, dF(c) \, dF(v)\\
        &= \frac{1}{2}\left(\int_{\beta_{\epsilon}}^{\beta_{1 - \epsilon}} \int_{\beta_{\epsilon}}^{\beta_{1 - \epsilon}} |v - c| \, dF(c) \, dF(v) + \iint_R |v - c| \, dF(c) \, dF(v)\right) \explain{where $R = \{(v, c) : v \not\in [\beta_{\epsilon}, \beta_{1 - \epsilon}] \lor c \not\in [\beta_{\epsilon}, \beta_{1 - \epsilon}]\}$}\\
        &= \frac{1}{2}\left(\int_{\beta_{\epsilon}}^{\beta_{1 - \epsilon}} \int_{\beta_{\epsilon}}^{\beta_{1 - \epsilon}} (\beta_{1 - \epsilon} - \beta_{\epsilon}) \, dF(c) \, dF(v) + \iint_R 1 \, dF(c) \, dF(v)\right)\\
        &\le \frac{1}{2}\left((1 - 2\epsilon)^2(\beta_{1 - \epsilon} - \beta_{\epsilon}) + (1 - (1 - 2\epsilon)^2)\right).
    \end{align*}
    But since
    \begin{align*}
        (\beta_{1 - \epsilon} - \beta_{\epsilon})\epsilon^2 &\le \Pro\\
        (\beta_{1 - \epsilon} - \beta_{\epsilon}) &\le \frac{\Pro}{\epsilon^2},
    \end{align*}
    we have that
    \begin{align*}
        \GFT^* &\le \frac{1}{2}\left(\frac{(1 - 2\epsilon)^2}{\epsilon^2}\Pro + (1 - (1 - 2\epsilon)^2)\right).
    \end{align*}
    Thus,
    \begin{align*}
        \frac{\GFT^*}{\GFT} &\le \frac{\GFT^*}{\Pro}\\
        &\le \frac{(1 - 2\epsilon)^2\Pro / \epsilon^2 + (1 - (1 - 2\epsilon)^2)}{2\Pro}\\
        &= \frac{(1 - 2\epsilon)^2}{2\epsilon^2} + \frac{(1 - (1 - 2\epsilon)^2)}{2\Pro}.
    \end{align*}
    Now, since $\Pro \le \GFT^* \le 1 / 4,$ taking $\epsilon = \Pro,$ 
    \begin{align*}
    \end{align*}
\end{proof}


\sscomment{Only problematic setting is, Profit is very small, $F(p_B)$ and $F(p_S)$ are both very small, then it suffices to prove that $\GFT^*$ is not that large.}

==> results.tex <==
\section{Results}
\allowdisplaybreaks
% \begin{comment}
\subsection{Approximation for the posted pricing mechanism}
\input{approx-ratio-by-percentiles}
    
\subsection{Inapproximability for the optimal mechanism}
\input{inapproximability_bounded}

\section{Gains-From-Trade in Restricted Settings}

\subsection{Uniform vs. Uniform}
\input{uniform}

\subsection{Singleton versus arbitrary distribution}
\input{singleton}

\subsection{Symmetric distributions}
\input{symmetric}


\subsection{Approximation for the Optimal Posted-Price Mechanism}
\input{optimal-posted-price}
% \end{comment}
% \subsection{$\lambda$-regular distribution}


==> singleton.tex <==
\subsubsection{Arbitrary Buyer, Singleton Seller}
In this section, we will study the case where $F$ is an arbitrary continuous distribution supported on $[a, b]$ and $G$ is singleton. We will first define some notation, adapted from~\cite{myerson1983efficient}.
\begin{definition}
    A \textit{direct mechanism} $(p, x_B, x_S)$ is characterized by three functions, $p(\cdot), x_B(\cdot),$ and $x_S(\cdot).$ Given that the buyer reports $v$ as his valuation, $p(v)$ is the probability that a trade occurs, $x_B(v)$ is the expected payment from the buyer to the intermediary, and $x_S(v)$ is the expected payment from the intermediary to the seller. (Since the seller's distribution is singleton, there is no need for the seller to report her valuation.) 
\end{definition}
\begin{definition}
    Given a direct mechanism $(p, x_B, x_S),$ we define the following functions for the expected utilities of the buyer, intermediary, and seller, respectively:
    \begin{itemize}
        \item $\displaystyle U_B(v) = vp(v) - x_B(v)$
        \item $\displaystyle U_I = \int_a^b (x_B(v) - x_S(v)) \, F'(v) \, dv$
        \item $\displaystyle U_S = \int_a^b (x_S(v) - cp(v)) \, F'(v) \, dv$
    \end{itemize}
\end{definition}
\begin{definition}
    We say that a direct mechanism $(p, x_B, x_S)$ is \textit{incentive-compatible} if $U_B(v) \ge vp(v') - x_B(v')$ for all $v, v'.$ We say that a direct mechanism is \textit{individually-rational} if $U_B(v) \ge 0$ for all $v$ and $U_S \ge 0.$
\end{definition}
By the revelation principle, any incentive-compatible mechanism can be simulated by an incentive-compatible direct mechanism, so we consider direct mechanisms without loss of generality, and we will henceforth simply refer to direct mechanisms as mechanisms.\\\\ 
The following theorems are analogues of Theorems 3 and 4, respectively, in~\cite{myerson1983efficient}:
\begin{theorem}
% \label{singleton-ic}
For any incentive-compatible mechanism $M = (p, x_B, x_S),$ $U_B(\cdot)$ is increasing and $$U_I + U_B(a) + U_S = \int_a^b \left(\left(v - \frac{1 - F(v)}{F'(v)}\right) - c\right) p(v) \, F'(v) \, dv.$$
\end{theorem}
\begin{proof}
Since $M$ is incentive-compatible, for any $v, v',$ $$U_B(v) = vp(v) - x_B(v) \ge vp(v') - x_B(v')$$ and $$U_B(v') = v'p(v') - x_B(v') \ge v'p(v) - x_B(v).$$ Thus, $$(v - v')p(v) \ge U_B(v) - U_B(v') \ge (v - v')p(v').$$ In particular, if $v > v',$ then $p(v) \ge p(v'),$ so $p(\cdot)$ is increasing and hence integrable. Therefore, $U'_B(v) = p(v)$ almost everywhere, so $$U_B(v) = U_B(a) + \int_a^v p(t) \, dt,$$ and $U_B(\cdot)$ is increasing.\\\\
Now, we have that
\begin{align*}
    \int_a^b (v - c)p(v) \, F'(v) \, dv - U_I &= \int_a^b (vp(v) - x_B(v)) \, F'(v) \, dv + \int_a^b (x_S(v) - cp(v)) \, F'(v) \, dv\\
    &= \int_a^b U_B(v)F'(v) \, dv + U_S\\
    &= \int_a^b \left(U_B(a) + \int_a^v p(t) \, dt\right)F'(v) \, dv + U_S\\
    &= U_B(a) + \int_a^b \int_a^v p(t) \, dt \, F'(v) \, dv + U_S\\
    &= U_B(a) + \int_a^b \int_t^b  F'(v) \, dv \, p(t) \, dt + U_S\\
    &= U_B(a) + \int_a^b (1 - F(t)) \, p(t) \, dt + U_S.
\end{align*}
From the first and last expressions in this chain of equalities, we obtain $$U_I + U_B(a) + U_S = \int_a^b \left(\left(v - \frac{1 - F(v)}{F'(v)}\right) - c\right) p(v) \, F'(v) \, dv.$$
\end{proof}
\begin{theorem}
    Suppose $\displaystyle\phi_F(v) = v - \frac{1 - F(v)}{F'(v)}$ is increasing. Then, among all incentive-compatible, individually-rational mechanisms, the intermediary's expected profit is maximized by a mechanism in which the object is transferred to the buyer if and only if $\phi_F(v) \ge c.$
\end{theorem}
\begin{proof}
By Theorem \ref{singleton-ic}, $$U_I = \int_a^b \left(\left(v - \frac{1 - F(v)}{F'(v)}\right) - c\right) p(v) \, F'(v) \, dv - U_B(a) - U_S.$$ Since we want an individually-rational mechanism $M = (p, x_B, x_S)$ that maximizes $U_I,$ we want $M$ to satisfy the following constraints:
\begin{itemize}
    \item $U_B(a) = 0$
    \item $U_S = 0$
    \item $p(v) = \begin{cases}
        1 & \text{if $\phi_F(v) \ge c$}\\
        0 & \text{otherwise}
    \end{cases}$
\end{itemize}
It remains to define $x_B(\cdot)$ and $x_S(\cdot)$ such that first two constraints are satisfied. We take $$x_B(v) = p(v) \cdot \min_{t \ge a, \phi_F(t) \ge c} t$$ and $$x_S(v) = p(v)c.$$ Since $x_B(a) = ap(a)$ and $x_S(v) - p(v)c = 0$ for all $v,$ we have that $U_B(a) = 0$ and $U_S = 0,$ as desired.\\\\
We leave it to the reader to verify that $M$ is incentive-compatible. (Note that if trade occurs, $x_B(v)$ is the lowest value the buyer could have bid and still have the trade occur.) Then, by Theorem \ref{singleton-ic}, $U_B(\cdot)$ is increasing, so since $U_B(a) = 0,$ $M$ is individually-rational.
\end{proof}
\begin{corollary}
% \label{singleton-seller-gft}
    Let $F$ be a continuous distribution supported on $[a, b]$ such that $\displaystyle\phi_F(v) = \frac{1 - F(v)}{F'(v)}$ is increasing, and let $G$ be a singleton distribution supported on $\{c\}.$ Then, the gains-from-trade from any incentive-compatible, individually-rational mechanism that maximizes the intermediary's expected profit is $$\int_a^b (v - c) \mathbf{1}\left\{v - c \ge \frac{1 - F(v)}{F'(v)}\right\}\, F'(v) \, dv.$$
\end{corollary}
We will now provide an example that shows that the ratio between the gains-from-trade of any incentive-compatible, individually-rational mechanism that maximizes the intermediary's expected profit and the optimal gains-from-trade can be arbitrarily close to $0.$
\begin{theorem}
    Let $\epsilon > 0.$ Then, there exists a continuous distribution $F$ with increasing $\displaystyle \phi_F(v) = v - \frac{1 - F(v)}{F'(v)}$ and a singleton distribution $G$ such that $\GFT < \epsilon\GFT^*,$ where $\GFT$ is the gains-from-trade of any incentive-compatible, individually-rational mechanism that maximizes the intermediary's expected profit and $\GFT^*$ is the gains-from-trade from an ex-post efficient mechanism.
\end{theorem}
\begin{proof}

Let $b > a > 0.$ Define 
\begin{align*}
F(v) = 
\begin{cases} 
    -\frac{a}{v} + 1 &\text{if $a \le v \le b$}\\
    \left(-\frac{a}{b} + 1\right) + \frac{a}{b^2}(v - b) &\text{if $b < v \le 2b$}
\end{cases}.
\end{align*}
Note that $F$ is differentiable on $(a, 2b)$ with $$F'(v) = 
\begin{cases} 
    \frac{a}{v^2} &\text{if $a < v \le b$}\\
    \frac{a}{b^2} &\text{if $b < v \le 2b$}
\end{cases}.$$
and that $\phi_F(v)$ is increasing. In addition, let $G$ be the singleton distribution supported on $\{a\}.$ Then, 
\begin{align*}
    \GFT^* &= \int_a^{2b} (v - a) \, F'(v) \, dv\\
    &= a\int_a^b \frac{v - a}{v^2} \, dv + \frac{a}{b^2}\int_b^{2b} (v - a) \, dv\\
    &= a\left[\ln v + \frac{a}{v}\right]_a^b + \frac{a}{b^2}\left[\frac{v^2}{2} - av\right]_b^{2b}\\
    &= a\left(\ln\left(\frac{b}{a}\right) + \frac{a}{b} - 1\right) + \left(\frac{3b^2}{2} - ab\right),
\end{align*}
and by Corollary~\ref{singleton-seller-gft},
\begin{align*}
    \GFT &= \int_a^{2b} (v - a)\mathbf{1}\left\{v - a \ge \frac{1 - F(v)}{F'(v)}\right\} \, F'(v) \, dv\\
    &= \frac{a}{b^2}\int_b^{2b} (v - a)\mathbf{1}\left\{v - a \ge \frac{1 - F(v)}{F'(v)}\right\} \, dv \explain{since $a > 0$ and $\displaystyle v = \frac{1 - F(v)}{F'(v)}$ on $(a, b)$ by construction}\\
    &= \frac{a}{b^2}\int_b^{2b} (v - a)\mathbf{1}\left\{v \ge \frac{a + 2b}{2}\right\}\, dv\\
    &= \frac{a}{b^2}\int_{a + 2b}^{2b} (v - a) \, dv \explain{since $\displaystyle b \le \frac{a + 2b}{2} \le 2b$ because $a > 0$ and $b > a$}\\
    &= \frac{a}{b^2}\left[\frac{v^2}{2} - av\right]_{a + 2b}^{2b}\\
    &= \frac{3a}{2} - \frac{a^3}{b^3}.
\end{align*}
Thus, as $b \rightarrow \infty,$ we have that $\GFT > 0$
but $\displaystyle\frac{\GFT}{\GFT^*} \rightarrow 0.$
\end{proof}
\subsubsection{Arbitrary Seller, Singleton Buyer}
We now study the case where $G$ is an arbitrary continuous distribution supported on $[a, b]$ and $F$ is singleton. Using similar ideas as those presented in the previous section, we leave it to the reader to prove the following theorem: 
\begin{theorem}
% \label{singleton-buyer-gft}
    Let $G$ be a continuous distribution supported on $[a, b]$ such that $\displaystyle\phi_G(v) = \frac{G(c)}{G'(c)}$ is increasing, and let $F$ be a singleton distribution supported on $\{v\}.$ Then, the gains-from-trade from any incentive-compatible, individually-rational mechanism that maximizes the intermediary's expected profit is $$\int_a^b (v - c) \mathbf{1}\left\{v - c \ge \frac{G(c)}{G'(c)}\right\}\, G'(c) \, dc.$$
\end{theorem}
As with the arbitrary-buyer, singleton-seller case, we have the following inapproximability result for the arbitrary-seller, singleton-buyer case:
\begin{theorem}
% \label{inapprox-singleton-sell}
    Let $\epsilon > 0.$ Then, there exists a continuous distribution $G$ with increasing $\displaystyle \phi_G(c) = c + \frac{G(c)}{G'(c)}$ and a singleton distribution $F$ such that $\GFT < \epsilon\GFT^*,$ where $\GFT$ is the gains-from-trade of any incentive-compatible, individually-rational mechanism that maximizes the intermediary's expected profit and $\GFT^*$ is the gains-from-trade from an ex-post efficient mechanism.
\end{theorem}
\begin{proof}
Let $\displaystyle 0 < \delta < \frac{1}{2}.$ Let
\begin{align*}
    G(c) &= \begin{cases}
        \delta c &\text{if $0 \le c \le 1$}\\
        h(c) &\text{if $1 < c \le 2$}
    \end{cases},
\end{align*}
where 
\begin{align*}
    h(c) &= k - \frac{a}{c - h}
\end{align*}
and
\begin{align*}
    h &= \frac{-2 + 3\delta}{-1 + 2\delta}\\
    a &= \delta(1 - h)^2\\
    k &= \delta(2 - h)
\end{align*}
are chosen so that
\begin{align*}
    h(1) &= \delta\\
    h'(1) &= \delta\\
    h(2) &= 1.
\end{align*}
It can be shown that $\phi_G(\cdot)$ is strictly increasing. Finally, let $F$ be the singleton distribution supported on $\{2\}.$\\\\
We have that
\begin{align*}
    \GFT^* &= \int_0^1 (2 - c)\delta \, dc + \int_1^2 (2 - c) \cdot \frac{a}{(c - h)^2} \, dc\\
    &= \delta\left[2c - \frac{c^2}{2}\right]_0^1 + a\left[\frac{h - 2}{c - h} - \ln(c - h)\right]_1^2\\
    &= \frac{3}{2}\delta + a\left(\frac{1}{1 - h} - \ln\left(\frac{2 - h}{1 - h}\right)\right)\\
    &= \frac{3}{2}\delta + \frac{\delta(1 - \delta)^2}{(2\delta - 1)^2}\left(\frac{2\delta - 1}{1 - \delta} - \ln\left(\frac{\delta}{1 - \delta}\right)\right)\\
    &\ge \frac{\delta(1 - \delta)^2}{(2\delta - 1)^2}\left(\frac{2\delta - 1}{1 - \delta} - \ln\left(\frac{\delta}{1 - \delta}\right)\right).
\end{align*}
In addition, by Theorem~\ref{singleton-buyer-gft}, the gains-from-trade for any incentive-compatible, individually-rational mechanism that maximizes the expected profit of the broker is given by
\begin{align*}
    \GFT &= \int_0^2 (2 - c) \mathbf{1}\left\{2 \ge c + \frac{G(c)}{G'(c)}\right\}\, G'(c) \, dc\\
    &= \int_0^1 (2 - c)\delta \, dc \explain{since $\phi_G(1) = 2$ and $\phi_G(\cdot)$ is strictly increasing}\\
    &= \frac{3}{2}\delta. \explain{from above}
\end{align*}
Thus,
\begin{align*}
    \frac{\GFT^*}{\GFT} \ge \frac{2(1 - \delta)^2}{3(2\delta - 1)^2}\left(\frac{2\delta - 1}{1 - \delta} - \ln\left(\frac{\delta}{1 - \delta}\right)\right),
\end{align*}
so taking the limit as $\delta \rightarrow 0,$ we obtain
\begin{align*}
    \lim_{\delta \rightarrow 0} \left(\frac{2(1 - \delta)^2}{3(2\delta - 1)^2}\left(\frac{2\delta - 1}{1 - \delta} - \ln\left(\frac{\delta}{1 - \delta}\right)\right)\right) &= \lim_{\delta \rightarrow 0} \frac{2(1 - \delta)}{3(2\delta - 1)} - \lim_{\delta \rightarrow 0} \frac{2(1 - \delta)^2}{3(2\delta - 1)^2} \ln \delta + \lim_{\delta \rightarrow 0} \frac{2(1 - \delta)^2}{3(2\delta - 1)^2} \ln (1 - \delta)\\
    &= -\frac{2}{3} - \lim_{\delta \rightarrow 0} \frac{2(1 - \delta)^2}{3(2\delta - 1)^2} \ln \delta\\
    &= \infty,
\end{align*}
which completes the proof.
\end{proof}


==> symmetric.tex <==
\sscomment{This can be motivated by size discovery mechanism, see \href{https://theory.stanford.edu/~jvondrak/data/Fixed-price-bilateral.pdf}{link}}
We now study the case where $F$ and $G$ are identical distributions. 
\begin{theorem}
Let $\epsilon > 0.$ Then, there exist identical distributions $F$ and $G$ with increasing $\displaystyle\phi_F(v) = v + \frac{1 - F(v)}{F'(v)}$ and increasing $\displaystyle\phi_G(c) = c + \frac{G(c)}{G'(c)}$ such that for any incentive-compatible, individually-rational mechanism that maximizes the expected profit for the broker, $$\GFT < \epsilon\GFT^*,$$ where $\GFT$ is the gains-from-trade of the mechanism and $\GFT^*$ is the gains-from-trade of any ex-post-efficient mechanism.
\end{theorem}
\begin{proof}
Let $b > a > 0.$ Consider the following distribution:
\begin{align*}
    F(v) &= 
    \begin{cases} 
        -\frac{a}{v} + 1 &\text{if $a \le v \le b$}\\
        \left(-\frac{a}{b} + 1\right) + \frac{a}{b^2}(v - b) &\text{if $b < v \le 2b$}
    \end{cases}
\end{align*}
Let $G = F.$ Note that both $\phi_F(\cdot)$ and $\phi_G(\cdot)$ are increasing.\\\\
We have that
\begin{align*}
    \GFT^* &= a^2\int_a^b \int_a^v (v - c) \, \frac{1}{c^2} \, dc \, \frac{1}{v^2} \, dv + \frac{a^2}{b^2}\int_b^{2b} \int_a^b (v - c) \, \frac{1}{c^2} \, dc \, dv + \frac{a^2}{b^4}\int_b^{2b} \int_b^v (v - c) \, dc \, dv\\
    &= a^2\int_a^b \left[-\frac{v}{c} - \ln c\right]_a^v \, \frac{1}{v^2} \, dv + \frac{a^2}{b^2}\int_b^{2b} \left[-\frac{v}{c} - \ln c\right]_a^b \, dv + \frac{a^2}{b^4}\int_b^{2b} \left[vc - \frac{c^2}{2}\right]_b^v \, dv\\
    &= a^2\int_a^b \left(\frac{v}{a} - 1 - \ln \left(\frac{v}{a}\right)\right) \, \frac{1}{v^2} \, dv + \frac{a^2}{b^2}\int_b^{2b} \left(\frac{v}{a} - \frac{v}{b} - \ln \left(\frac{b}{a}\right)\right) dv + \frac{a^2}{2b^4}\int_b^{2b} (v - b)^2 \, dv\\
    &= a^2\left[\frac{1}{a} \ln v + \frac{1}{v} + \frac{1}{v}\left(\ln \left(\frac{v}{a}\right) + 1\right) \right]_a^b + \frac{a^2}{b^2}\left[\frac{v^2}{2a} - \frac{v^2}{2b} - v\ln \left(\frac{b}{a}\right)\right]_b^{2b} + \frac{a^2}{2b^4}\left[\frac{(v - b)^3}{3}\right]_b^{2b}\\
    &= a^2\left(\frac{1}{a}\ln\left(\frac{b}{a}\right) + \left(\frac{1}{b} - \frac{1}{a}\right) + \frac{1}{b}\left(\ln\left(\frac{b}{a}\right) + 1\right) - \frac{1}{a}\right) + \frac{a^2}{b^2}\left(\frac{3b^2}{2a} - \frac{3b}{2} - b\ln\left(\frac{b}{a}\right)\right) + \frac{a^2}{2b^4}\left(\frac{b^3}{3}\right)\\
    &= \left(a\ln\left(\frac{b}{a}\right) + \left(\frac{a^2}{b} - a\right) + \frac{a^2}{b}\left(\ln\left(\frac{b}{a}\right) + 1\right) - a\right) + \left(\frac{3a}{2} - \frac{3a^2}{2b} - \frac{a^2}{b}\ln\left(\frac{b}{a}\right)\right) + \frac{a^2}{6b}
\end{align*}
In addition, by~\cite{myerson1983efficient}, the gains-from-trade of any incentive-compatible, individually-rational mechanism that maximizes the expected profit of the broker is given by
\begin{align*}
    \GFT &= \iint (v - c)\mathbf{1}\left\{v - c \ge \frac{1 - F(v)}{F'(v)} + \frac{G(c)}{G'(c)}\right\} \, F'(v) \, dv \, G'(c) \, dc\\
    &= \frac{a}{b^2}\int_b^{2b} \int (v - c)\mathbf{1}\left\{v - c \ge (2v - 2b) + \frac{G(c)}{G'(c)}\right\} \, G'(c) \, dc \, dv \explain{since $\displaystyle v = \frac{1 - F(v)}{F'(v)}$ on $(a, b)$ and $c > 0$}\\
    &= \frac{a^2}{b^2}\int_b^{2b} \int_a^b (v - c)\mathbf{1}\left\{v - c \ge (2v - 2b) + \frac{c^2}{a}\right\} \frac{1}{c^2} \, dc \, dv\\
    &+ \frac{a^2}{b^4}\int_b^{2b} \int_b^{2b} (v - c)\mathbf{1}\left\{v - c \ge (2v - 2b) + \left(2c - 2b + \frac{b^2}{a}\right)\right\} \, dc \, dv\\
    &\le \frac{a^2}{b^2}\int_b^{2b} \int_a^b (v - c)\frac{1}{c^2} \, dc \, dv + \frac{a^2}{b^4}\int_b^{2b} \int_b^{2b} (v - c)\mathbf{1}\left\{c \le \frac{4b - v - b^2 / a}{3}\right\} \, dc \, dv\\
    &= \frac{a^2}{b^2}\int_b^{2b} \int_a^b (v - c)\frac{1}{c^2} \, dc \, dv \explain{since $\displaystyle\frac{4b - v - b^2 / a}{3} < b$ whenever $v \in [b, 2b]$}\\
    &= \frac{3a}{2} - \frac{3a^2}{2b} - \frac{a^2}{b}\ln\left(\frac{b}{a}\right) \explain{from calculations above}.
\end{align*}
Thus, since $\displaystyle\GFT \sim \frac{3a}{2}$ and $\displaystyle\GFT^* \sim a \ln\left(\frac{b}{a}\right)$ as $b \rightarrow \infty,$ we have that $\displaystyle\frac{\GFT}{\GFT^*} \rightarrow 0$ as $b \rightarrow \infty.$
\end{proof}


==> uniform.tex <==
Let $F, G$ be the the cumulative distributions for the buyer's value and seller's cost, respectively. Furthermore, let $[a_1, b_1]$ and $[a_2, b_2]$ be the supports of $F$ and $G,$ respectively, and suppose $\phi_F$ and $\phi_G$ are monotonically increasing. 
\sscomment{What if the supports are union of disjoint intervals? Not saying this would be worth exploring, but just wonder if a simple argument would reduce the burden for such case as well. Seems the Myerson and Satterthwaite also focuses on continuums so probably fine}
By~\cite{myerson1983efficient}, the gains-from-trade for any incentive-compatible, individually-rational mechanism that maximizes the broker's profit is given by $$\GFT_{F, G} = \int_{a_2}^{b_2} \int_{a_1}^{b_1} (v - c)\mathbf{1}\left\{v - c \ge \frac{1 - F(v)}{F'(v)} + \frac{G(c)}{G'(c)}\right\} F'(v) \, dv \; G'(c) \, dc.$$ As usual, the optimal gains-from-trade is given by $$\GFT^*_{F, G} =\int_{a_2}^{b_2} \int_{a_1}^{b_1} (v - c)\mathbf{1}\left\{v - c \ge 0\right\} F'(v) \, dv \; G'(c) \, dc.$$\\
We first prove a lemma that will simplify our analysis. The lemma states that the approximability factor of the optimal mechanism for the broker is invariant to stretches and shifts in $F$ and $G,$ provided that we perform the same stretches and shifts to $F$ and $G.$

\sscomment{regularity condition (the assumption imposed on~\cite{myerson1983efficient}) should be assumed? and also regularity carries over to these transformations? For non-regular case, \cite{myerson1983efficient} discussed one can use Myerson's ironing, so the argument still carries over.}
\begin{lemma} Let $F^*(v) = F((v - k_1) / k_2)$ and $G^*(c) = G((c - k_1) / k_2)$ for $k_1, k_2 \in \mathbb{R}$ and $k_2 > 0.$ If $\GFT_{F, G} = \alpha\GFT^*_{F, G},$ then $\GFT_{F', G'} = \alpha\GFT^*_{F', G'}.$
\end{lemma}
\begin{proof}
Note that the supports of $F^*, G^*$ are $[a_1^*, b_1^*] = [k_2a_1 + k_1, k_2b_1 + k_1]$ and $[a_2^*, b_2^*] = [k_2a_2 + k_1, k_2b_2 + k_1],$ respectively. Substituting $v^* = k_2v + k_1$ and $c^* = k_2c + k_1$ into the expression for $\GFT_{F, G},$ we obtain
\begin{align*}
    \GFT_{F, G} &= \int_{a_2}^{b_2} \int_{a_1}^{b_1} (v - c)\mathbf{1}\left\{v - c \ge \frac{1 - F(v)}{F'(v)} + \frac{G(c)}{G'(c)}\right\} F'(v) \, dv \; G'(c) \, dc\\
    &= \int_{a^*_2}^{b^*_2} \int_{a^*_1}^{b^*_1} \frac{v^* - c^*}{k_2}\mathbf{1}\left\{\frac{v^* - c^*}{k_2} \ge \frac{1 - F(\frac{v^* - k_1}{k_2})}{F'(\frac{v^* - k_1}{k_2})} + \frac{G(\frac{c^* - k_1}{k_2})}{G'(\frac{c^* - k_1}{k_2})}\right\} \frac{1}{k_2}F'(v^*) \, dv^* \; \frac{1}{k_2} \; G'(c^*) \, dc^*\\
    &= \frac{1}{k_2}\int_{a^*_2}^{b^*_2} \int_{a^*_1}^{b^*_1} (v^* - c^*)\mathbf{1}\left\{v^* - c^* \ge \frac{1 - (F*)'(v)}{(F^*)'(v^*)} + \frac{(G^*)'(c)}{(G^*)'(c^*)}\right\} (F^*)'(v^*) \, dv^* \; (G^*)'(c^*) \, dc^*\\
    &= \frac{1}{k_2}\GFT_{F', G'}.
\end{align*}
\sscomment{perhaps better to mention that $(F^*)' = k_2 \cdot F'$}
A similar argument will show that $$\GFT^*_{F, G} = \frac{1}{k_2}\GFT^*_{F^*, G^*}.$$ Thus, if $\GFT_{F, G} = \alpha\GFT^*_{F, G},$ then $$\GFT_{F^*, G^*} = k_2\GFT_{F, G} = \alpha k_2\GFT^*_{F, G} = \alpha\GFT^*_{F^*, G^*}.$$
\end{proof}
It directly follows from the above theorem that we can assume $[a_1, b_1] = [0, 1]$ without loss of generality.
Let $F, G$ be the uniform distributions on $[0, 1]$ and $[a, b],$ respectively, i.e., let $$F(v) = \begin{cases} v &\text{if $v \in [0, 1]$}\\ 0 &\text{otherwise}\end{cases}$$ and $$ G(c) = \begin{cases} \displaystyle\frac{c - a}{b - a} &\text{if $c \in [a, b]$}\\ 0 &\text{otherwise}\end{cases}$$
Note that $\phi_F(v)$ and $\phi_G(c)$ are both monotonically increasing. By~\cite{myerson1983efficient},
\begin{align*}
    \GFT &= \iint (v - c)\left\{v - c \ge \frac{1 - F(v)}{F'(v)} + \frac{G(c)}{G'(c)}\right\} \, F'(v) \, dv \; G'(c) \, dc\\
    &= \iint (v - c)\left\{v - c \ge (1 - v) + (c - a) \right\} \, F'(v) \, dv \; G'(c) \, dc,\\
    &= \iint (v - c)\left\{v - c \ge T_a \right\} \, F'(v) \, dv \; G'(c) \, dc,
\end{align*}
where $\displaystyle T_a = \frac{1 - a}{2}.$\\\\
The following two tables will be helpful for our analysis:
\begin{center}
    \renewcommand{\arraystretch}{2}
    \begin{tabular}{|c|c|c|c|}
        \hline
        & $\GFT^*$ & Case & Derivation\\
        \hline
        $b \le 0$ & $\displaystyle\frac{1 - a - b}{2}$ & 1 & $\hyperref[sec:derivations]{1}$\\ 
        \hline
        $a \le 0 < b \le 1$ & $\displaystyle\frac{3a^2 - 3a + b^3 - 3b^2 + 3b}{6(b - a)}$ & 2 & $\hyperref[sec:derivations]{2}$\\
        \hline
        $a \le 0 < 1 < b$ & $\displaystyle\frac{3a^2 - 3a + 1}{6(b - a)}$ & 3 & $\hyperref[sec:derivations]{3}$\\
        \hline
        $0 < a < b \le 1$ & $\displaystyle\frac{a^2 + ab + b^2 - 3a - 3b + 3}{6}$ & 4 & $\hyperref[sec:derivations]{4}$\\
        \hline
        $0 < a < 1 < b$ & $\displaystyle\frac{(1 - a)^3}{6(b - a)}$ & 5 & $\hyperref[sec:derivations]{5}$\\
        \hline
    \end{tabular}
\end{center}
\begin{center}
    \renewcommand{\arraystretch}{2}
    \begin{tabular}{|c|c|c|c|}
        \hline
        & $\GFT$ & Subcase & Derivation\\
        \hline
        $b + T_a \le 0$ & $\displaystyle\frac{1 - a - b}{2}$ & $(a)$ & $\hyperref[sec:derivations]{1}$\\ 
        \hline
        $a + T_a \le 0 < b + T_a \le 1$ & $\displaystyle\frac{(a + b - 1)(a^2 - 4ab + 10a + 4b^2 - 8b + 1)}{24(b - a)}$ & $(b)$ & $\hyperref[sec:derivations]{6}$\\
        \hline
        $a + T_a \le 0 < 1 < b + T_a$ & $\displaystyle\frac{(3a - 1)^2}{24(b - a)}$ & $(c)$ & $\hyperref[sec:derivations]{7}$\\
        \hline
        $0 < a + T_a < b + T_a \le 1$ & $\displaystyle\frac{(a + 2b - 3)^2}{24}$ & $(d)$ & $\hyperref[sec:derivations]{8}$\\
        \hline
        $0 < a + T_a \le 1 < b + T_a$ & $\displaystyle \frac{(1 - a)^3}{12(b - a)}$ & $(e)$ & $\hyperref[sec:derivations]{9}$\\
        \hline
    \end{tabular}
\end{center}
\ \\
The table below summarizes the results of our analysis:
\begin{table}
    \centering
    \renewcommand{\arraystretch}{1.5}
    \begin{tabular}{|c|c|c|c|c|c|}
        \hline
        \multicolumn{6}{|c|}{Summary of Lower Bounds on Efficiency}\\
        \hline
        & \multicolumn{5}{c|}{Subcase}\\
        \hline
        Case & $(a)$ & $(b)$ & $(c)$ & $(d)$ & $(e)$\\
        \hline
        1 & $\hyperref[sec:1a]{1}$ & $\hyperref[sec:1b]{2 / 3}$ & $\hyperref[sec:1c]{2 / 3}$ & $\hyperref[sec:1d]{2 / 3}$ &\\
        \hline
        2 & & & $\hyperref[sec:2c]{4 / 7}$ & $\hyperref[sec:2d]{4 / 7}$ & $\hyperref[sec:2e]{1 / 2}$\\
        \hline
        3 & & & $\hyperref[sec:3c]{4 / 7}$ & & $\hyperref[sec:3e]{1 / 2}$\\
        \hline
        4 & & & & $\hyperref[sec:4d]{4 / 7}$ & $\hyperref[sec:4e]{1 / 2}$\\
        \hline
        5 & & & & & $\hyperref[sec:5e]{1 / 2}$\\
        \hline
    \end{tabular}
    \caption{Empty cell denotes that the corresponding case is not possible.}
\end{table}
In fact, the lower bounds above are tight:
\begin{table}
\centering
    \renewcommand{\arraystretch}{1.5}
    \begin{tabular}{|c|c|c|c|c|c|}
        \hline
        % \multicolumn{6}{|c|}{}\\
        % \hline
        & \multicolumn{5}{c|}{Subcase}\\
        \hline
        Case & $(a)$ & $(b)$ & $(c)$ & $(d)$ & $(e)$\\
        \hline
        1 & $[-3, -2]$ & $[-1, 0]$ & $[-1 - \epsilon, 0]$ & $[-1 + \epsilon, 0]$ &\\
        \hline
        2 & & & $[-1, 1]$ & $[0, 1/2]$ & $[0, 1]$\\
        \hline
        3 & & & $[-1, 2]$ & & $[0, 2]$\\
        \hline
        4 & & & & $[1 / 3, 2 / 3]$ & $[1 / 2, 1]$\\
        \hline
        5 & & & & & $[1 / 2, 3 / 2]$\\
        \hline
    \end{tabular}
    \caption{Example Values of $a$ and $b$ that Match Above Lower Bounds. $-$ denotes that the corresponding case is not possible. }
\end{table}
\sscomment{You can consider using nicefrac for inline frac, which is often more visible.}
\ \\
Thus, we have the following theorem:
\begin{theorem}
    If $F$ and $G$ are uniform distributions, then the worst-case approximation ratio of the gains-from-trade for any incentive-compatible, individually-rational mechanism that maximizes the broker's expected profit is $\nicefrac{1}{2}.$ Furthermore, this bound is tight \ssedit{in a sense that there exists a problem instance in which the optimal GFT is exactly $\nicefrac{1}{2}$.}
\end{theorem}
\begin{proof}
\sscomment{Could you first start with justifying why the following cases are sufficient to deal with? Or a brief proof sketch would be great.}
\medskip
\sscomment{Instead of four backslashes, you can use medskip and noindent}

Due to Lemma~\ref{lem:invariance}, we can assume $[a_1, b_1] = [0, 1]$ without loss of generality.
Let $F, G$ be the uniform distributions on $[0, 1]$ and $[a, b],$ respectively.
\Ie let $$F(v) = \begin{cases} v &\text{if $v \in [0, 1]$}\\ 0 &\text{otherwise}\end{cases}$$ and $$ G(c) = \begin{cases} \displaystyle\frac{c - a}{b - a} &\text{if $c \in [a, b]$}\\ 0 &\text{otherwise}\end{cases}$$
It is straightforward to check that $\phi_F(v)$ and $\phi_G(c)$ are both monotonically increasing. By~\cite{myerson1983efficient},
\begin{align*}
    \GFT &= \iint (v - c)\left\{v - c \ge \frac{1 - F(v)}{F'(v)} + \frac{G(c)}{G'(c)}\right\} \, dF(v) dG(c)\\
    &= \iint (v - c)\left\{v - c \ge (1 - v) + (c - a) \right\} \, dF(v) dG(c)\\
    &= \iint (v - c)\left\{v - c \ge T_a \right\} \, dF(v)dG(c),
\end{align*}
where $ T_a = \frac{1 - a}{2}$.



\paragraph{Case 1: $b \le 0$}

\medskip \noindent \textit{Case 1(a):} $b + T_a \le 0$\\\\
\label{sec:1a}We have that $$\GFT = \frac{1 - a - b}{2} = \GFT^*.$$\\\\
\textit{Case 1(b):} $a + T_a \le 0 < b + T_a \le 1$\\\\
\label{sec:1b}We seek to lower bound $$\frac{\GFT}{\GFT^*} = \frac{-a^2 + 4ab - 10a - 4b^2 + 8b - 1}{12(b - a)}$$ subject to
\begin{align*}
    a + T_a &\le 0\\
    a &\le -1
\end{align*}
and
\begin{align*}
    0 &\le b + T_a \le 1\\
    \frac{a - 1}{2} &\le b \le \frac{a + 1}{2}.
\end{align*}
Taking the derivative with respect to $b,$ we obtain
\begin{align*}
    \frac{\partial}{\partial b}\left[\frac{-a^2 + 4ab - 10a - 4b^2 + 8b - 1}{12(b - a)}\right] &= \frac{12(b - a)(4a - 8b + 8) - 12(-a^2 + 4ab - 10a - 4b^2 + 8b - 1)}{(12(b - a))^2}\\
    &= \frac{(4ab - 8b^2 + 8b - 4a^2 + 8ab - 8a) + (a^2 - 4ab + 10a + 4b^2 - 8b + 1)}{12(b - a)^2}\\
    &= \frac{8ab - 4b^2 - 3a^2 + 2a + 1}{12(b - a)^2}\\
    &= \frac{(-a + 2b + 1)(3a - 2b + 1)}{12(b - a)^2}.
\end{align*}
Now, since $-a + 2b + 1 \ge 0$ and $3a - 2b + 1 \le 0$ whenever $a \in (-\infty, -1]$ and $\displaystyle b \in \left[\frac{a - 1}{2}, \frac{a + 1}{2}\right],$ $\displaystyle\frac{\GFT}{\GFT^*}$ is an decreasing function with respect to $b$ on $a \in (-\infty, -1]$ and $\displaystyle b \in \left[\frac{a - 1}{2}, \frac{a + 1}{2}\right].$ Thus,
\begin{align*}
    \frac{\GFT}{\GFT^*} &= \frac{-a^2 + 4ab - 10a - 4b^2 + 8b - 1}{12(b - a)}\\
    &\ge \frac{-a^2 + (2a^2 + 2a) - 10a - (a^2 + 2a + 1) + (4a + 4) - 1}{6 - 6a}\\
    &= \frac{2 - 6a}{6 - 6a}\\
    &\ge \frac{2 - 6(-1)}{6 - 6(-1)} \explain{since $a \le -1$}\\
    &= \frac{2}{3}.
\end{align*}
\ \\
\textit{Case 1(c):} $a + T_a \le 0 < 1 < b + T_a$\\\\
\label{sec:1c}We have that
\begin{align*}
    \frac{\GFT}{\GFT^*} &= \frac{(3a - 1)^2}{12(b - a)(1 - a - b)}\\
    &\ge \frac{(3a - 1)^2}{12a(a - 1)} \explain{since $(b - a)(1 - a - b)$ is increasing on $(\infty, 0]$}\\
    &\ge \frac{2}{3} \explain{since $\frac{(3a - 1)^2}{12\left(1 / 2 - a\right)^2}$ is decreasing on $(-\infty, -1]$}.\\ 
\end{align*}
\ \\
\textit{Case 1(d):} $0 < a + T_a < b + T_a \le 1$\\\\
\label{sec:1d}We seek to lower bound $$\frac{\GFT}{\GFT^*} = \frac{(a + 2b - 3)^2}{12(1 - a - b)}$$ subject to 
\begin{align*}
    a + T_a &\ge 0\\
    a &\ge -1.
\end{align*}
Taking the derivative with respect to $b,$ we obtain
\begin{align*}
    \frac{\partial}{\partial b}\left[\frac{(a + 2b - 3)^2}{12(1 - a - b)}\right] &= \frac{48(1 - a - b)(a + 2b - 3) + 12(a + 2b - 3)^2}{(12(1 - a - b))^2}\\
    &= \frac{(a + 2b - 3)(1 - 3a - 2b)}{12(1 - a - b)^2}.
\end{align*}
Thus, since $$a + 2b - 3 \le -3$$ and $$1 - 3a - 2b \ge 1$$ whenever $a, b \in [-1, 0],$ we have that $ \frac{\GFT}{\GFT^*}$ is decreasing with respect to $b$ on $a, b \in [-1, 0]$ Hence,
\begin{align*}
    \frac{\GFT}{\GFT^*} &= \frac{(a + 2b - 3)^2}{12(1 - a - b)}\\
    &\ge \frac{(a - 3)^2}{12(1 - a)}\\
    &\ge \frac{2}{3}. \explain{since $\displaystyle\frac{(a - 3)^2}{12(1 - a)}$ is increasing on $[-1, 0]$}
\end{align*}
\ \\
\textit{Case 1(e):} $0 < a + T_a \le 1 < b + T_a$\\\\
Since
\begin{align*}
    a + T_a &> 0\\
    a &> -1,
\end{align*}
we have that
\begin{align*}
    b + T_a &> 1\\
    b &> \frac{a + 1}{2} > 0,
\end{align*}
so this case is impossible.\\\\
\textbf{Case 2:} $a \le 0 < b \le 1$\\\\
\textit{Case 2(a):} $b + T_a \le 0$\\\\
Since $T_a > 0$ and $b > 0,$ this case is impossible.\\\\
\textit{Case 2(b):} $a + T_a \le 0 < b + T_a \le 1$\\\\
Since 
\begin{align*}
    a + T_a &\le 0\\
    a &\le -1
\end{align*}
and $$b + T_a \le 1,$$ we have that $$b \le \frac{a + 1}{2} \le 0,$$ so this case is impossible.\\\\
\textit{Case 2(c):} $a + T_a \le 0 < 1 < b + T_a$\\\\
\label{sec:2c}We seek to lower bound
\begin{align*}
    \frac{\GFT}{\GFT^*} &= \frac{(3a - 1)^2}{4(3a^2 - 3a + b^3 - 3b^2 + 3b)}\\
    &\ge \frac{(3a - 1)^2}{4(3a^2 - 3a + 1)} \explain{since $b^3 - 3b^2 + 3b$ is increasing on $[0, 1]$}\\
    &\ge \frac{4}{7} \explain{since $\displaystyle\frac{(3a - 1)^2}{4(3a^2 - 3a + 1)}$ is decreasing on $(-\infty, -1]$}.
\end{align*}
\ \\
\textit{Case 2(d):} $0 < a + T_a < b + T_a \le 1$\\\\
\label{sec:2d}We seek to lower bound $$\frac{\GFT}{\GFT^*} = \frac{(a + 2b - 3)^2(b - a)}{4(3a^2 - 3a + b^3 - 3b^2 + 3b)}.$$ Taking the derivative with respect to $b,$ we obtain
\begin{align*}
    \frac{\partial}{\partial b}\left[\frac{(a + 2b - 3)^2(b - a)}{4(3a^2 - 3a + b^3 - 3b^2 + 3b)}\right] &= \frac{4(3a^2 - 3a + b^3 - 3b^2 + 3b)(4(a + 2b - 3)(b - a) + (a + 2b - 3)^2)}{(4(3a^2 - 3a + b^3 - 3b^2 + 3b))^2}\\
    &- \frac{4(a + 2b - 3)^2(b - a)(3b^2 - 6b + 3)}{(4(3a^2 - 3a + b^3 - 3b^2 + 3b))^2}\\
    &= -\frac{12(3a^2 - 3a + b^3 - 3b^2 + 3b)(a + 2b - 3)(a - 2b + 1)}{(4(3a^2 - 3a + b^3 - 3b^2 + 3b))^2}\\
    &- \frac{12(a + 2b - 3)^2(b - a)(b - 1)^2}{(4(3a^2 - 3a + b^3 - 3b^2 + 3b))^2}\\
    &= -\frac{12(a + 2b - 3)}{(4(3a^2 - 3a + b^3 - 3b^2 + 3b))^2}((3a^2 - 3a + b^3 - 3b^2 + 3b)(a - 2b + 1)\\ 
    &+ (a + 2b - 3)(b - a)(b - 1)^2)\\
    &= -\frac{12(a + 2b - 3)}{(4(3a^2 - 3a + b^3 - 3b^2 + 3b))^2}\\
    &((3a^3 + ab^3 - 3ab^2 + 9ab - 6a^2b - 2b^4 + 7b^3 - 9b^2 - 3a + 3b)\\
    &+ (-ab^3 + 2b^4 - 7b^3 - a^2b^2 + 5ab^2 + 8b^2 + 2a^2b - 7ab - 3b - a^2 + 3a))\\
    &= -\frac{12(a + 2b - 3)}{(4(3a^2 - 3a + b^3 - 3b^2 + 3b))^2}(3a^3 + 2ab^2 + 2ab - 4a^2b - b^2 - a^2b^2 - a^2)
\end{align*}
Now, since $a \le 0$ and $b \ge 0,$ each of the terms in the rightmost factor is nonpositive. In addition, since $a \le 0$ and 
\begin{align*}
    b + T_a \le 1\\
    b \le \frac{a + 1}{2},
\end{align*}
we have that $a + 2b - 3 \le 0.$ Thus,
$\displaystyle\frac{(a + 2b - 3)^2(b - a)}{4(3a^2 - 3a + b^3 - 3b^2 + 3b)}$ is decreasing with respect to $b$ on $a \in [-1, 0]$ and $\displaystyle b \in \left[0, \frac{a + 1}{2}\right].$ Hence,
\begin{align*}
    \frac{\GFT}{\GFT^*} &\ge \frac{(2a - 2)^2((1 - a) / 2)}{4(3a^2 - 3a + (a^3 - 3a^2 + 3a + 7) / 8)}\\
    &= \frac{4(a - 1)^2(1 - a)}{24a^2 - 24a + (a^3 - 3a^2 + 3a + 7)}\\
    &= \frac{4(1 - a)^3}{a^3 + 21a^2 - 21a + 7}.
\end{align*}
Taking the derivative, we obtain
\begin{align*}
    \frac{d}{da}\left[\frac{4(1 - a)^3}{a^3 + 21a^2 - 21a + 7}\right] &= \frac{-12(1 - a)^2(a^3 + 21a^2 - 21a + 7) - 4(1 - a)^3(3a^2 + 42a - 21)}{(a^3 + 21a^2 - 21a + 7)^2}\\
    &= -\frac{96(1 - a)^2a^2}{(a^3 + 21a^2 - 21a + 7)^2},
\end{align*}
so $\displaystyle\frac{4(1 - a)^3}{a^3 + 21a^2 - 21a + 7}$ is decreasing on $[-1, 0].$ Therefore, $$\frac{\GFT}{\GFT^*} \ge \frac{4}{7}.$$
\ \\
\textit{Case 2(e):} $0 < a + T_a \le 1 < b + T_a$\\\\
\label{sec:2e}We have that
\begin{align*}
    \frac{\GFT}{\GFT^*} &= \frac{(1 - a)^3}{2(3a^2 - 3a + b^3 - 3b^2 + 3b)}\\
    &\ge \frac{(1 - a)^3}{2(3a^2 - 3a + 1)} \explain{since $b^3 - 3b^2 + 3b$ is increasing on $[0, 1]$}\\
    &\ge \frac{1}{2} \explain{since $\displaystyle\frac{(1 - a)^3}{2(3a^2 - 3a + 1)}$ is decreasing on $[-1, 0]$}
\end{align*}
\ \\
\textbf{Case 3:} $a \le 0 < 1 < b$\\\\
\textit{Cases 3(a), (b), (d):} $b + T_a \le 1$\\\\
Since $b > 1$ and $T_a > 0,$ this case is impossible.\\\\
\textit{Case 3(c):} $a + T_a \le 0 < 1 < b + T_a$\\\\
\label{sec:3c}We have that
\begin{align*}
    \frac{\GFT}{\GFT^*} &= \frac{(3a - 1)^2}{4(3a^2 - 3a + 1)}\\
    &\ge \frac{4}{7}. \explain{since $\displaystyle\frac{(3a - 1)^2}{4(3a^2 - 3a + 1)}$ is decreasing on $(-\infty, -1]$}
\end{align*}
\ \\
\textit{Case 3(e):} $0 < a + T_a \le 1 < b + T_a$\\\\
\label{sec:3e}We have that
\begin{align*}
    \frac{\GFT}{\GFT^*} &= \frac{(1 - a)^3}{2(3a^2 - 3a + 1)}\\
    &\ge \frac{1}{2}. \explain{since $\displaystyle\frac{(1 - a)^3}{2(3a^2 - 3a + 1)}$ is decreasing on $[-1, 0]$}
\end{align*}
\ \\
\textbf{Case 4:} $0 < a < b \le 1$\\\\
\textit{Case 4(a):} $b + T_a \le 0$\\\\
Since $b > 0$ and $T_a > 0,$ this case is impossible.\\\\
\textit{Cases 4(b), (c):} $a + T_a \le 0$\\\\
Since $a > 0$ and $T_a > 0,$ this case is impossible.\\\\
\textit{Case 4(d):} $0 < a + T_a < b + T_a \le 1$\\\\
\label{sec:4d}We seek to minimize $$\frac{\GFT}{\GFT^*} = \frac{(a + 2b - 3)^2}{4(a^2 + ab + b^2 - 3a - 3b + 3)}.$$ Taking the derivative with respect to $b,$
\begin{align*}
    \frac{\partial}{\partial b}\left[\frac{(a + 2b - 3)^2}{4(a^2 + ab + b^2 - 3a - 3b + 3)}\right] &= \frac{16(a^2 + ab + b^2 - 3a - 3b + 3)(a + 2b - 3) - 4(a + 2b - 3)^3}{(4(a^2 + ab + b^2 - 3a - 3b + 3))^2}\\
    &= \frac{12(a + 2b - 3)(a - 1)^2}{(4(a^2 + ab + b^2 - 3a - 3b + 3))^2}.
\end{align*}
Now, since $a, b \le 1,$ we have that $a + 2b - 3 \le 0,$ so $\displaystyle\frac{(a + 2b - 3)^2}{4(a^2 + ab + b^2 - 3a - 3b + 3)}$ is decreasing with respect to $b$ on $a \in [0, 1]$ and $\displaystyle b \in \left[0, \frac{a + 1}{2}\right].$ Thus,
\begin{align*}
    \frac{\GFT}{\GFT^*} &\ge \frac{(2a - 2)^2}{4a^2 + 2a(a + 1) + (a^2 + 2a + 1) - 12a - 6(a + 1) + 12)}\\
    &= \frac{(2a - 2)^2}{7(a - 1)^2}\\
    &= \frac{4}{7}.
\end{align*}
\ \\
\textit{Case 4(e):} $0 < a + T_a \le 1 < b + T_a$\\\\
\label{sec:4e}We seek to lower bound $$\frac{\GFT}{\GFT^*} = \frac{(1 - a)^3}{2(b - a)(a^2 + ab + b^2 - 3a - 3b + 3)}.$$ Taking the derivative of the denominator with respect to $b,$ we obtain 
\begin{align*}
    \frac{\partial}{\partial b}[2(b - a)(a^2 + ab + b^2 - 3a - 3b + 3)] &= 2(b - a)(2b + a - 3) + 2(a^2 + ab + b^2 - 3a - 3b + 3)\\
    &= 2(2b^2 - ab - 3b - a^2 + 3a) + 2(a^2 + ab + b^2 - 3a - 3b + 3)\\
    &= 6b^2 - 12b + 6\\
    &= 6(b - 1)^2,
\end{align*}
so $2(b - a)(a^2 + ab + b^2 - 3a - 3b + 3)$ is increasing on $[0, 1].$ Thus,
\begin{align*}
    \frac{\GFT}{\GFT^*} &= \frac{(1 - a)^3}{2(b - a)(a^2 + ab + b^2 - 3a - 3b + 3)}\\
    &\ge \frac{(1 - a)^3}{2(1 - a)(a^2 - 2a + 1)}\\
    &= \frac{1}{2}.
\end{align*}
\ \\
\textbf{Case 5:} $0 < a < 1 < b$\\\\
\textit{Cases 5(a), (b), (d):} $b + T_a \le 1$\\\\
Since $b > 1$ and $T_a > 0,$ this case is impossible.\\\\
\textit{Case 5(c):} $a + T_a \le 0$\\\\
Since $a > 0$ and $T_a > 0,$ this case is impossible.\\\\
\textit{Case 5(e):} $0 < a + T_a \le 1 < b + T_a$\\\\
\label{sec:5e}We have that $$\frac{\GFT}{\GFT^*} = \frac{1}{2}.$$\\
\textbf{Case 6:} $a > 1$\\\\
We have that $\GFT = 0 = \GFT^*.$
\end{proof}
\subsubsection{Derivations}
\label{sec:derivations}
\begin{enumerate}
    \item \begin{align*}
    \frac{1}{b - a}\int_0^1 \int_a^b (v - c) \, dc \, dv &= \frac{1}{b - a}\int_0^1 \left[vc - \frac{c^2}{2}\right]_a^b \, dv\\
    &= \frac{1}{b - a}\int_0^1 \left(v(b - a) - \frac{b^2 - a^2}{2}\right) \, dv\\
    &= \int_0^1 \left(v - \frac{a + b}{2}\right) \, dv\\
    &= \int_0^1 \left[\frac{v^2}{2} - \frac{(a + b)v}{2}\right]_0^1\\
    &= \frac{1 - a - b}{2}
    \end{align*}
    \item \begin{align*}
        &\frac{1}{b - a}\int_0^b \int_a^v (v - c) \, dc \, dv + \frac{1}{b - a}\int_b^1 \int_a^b (v - c) \, dc \, dv\\
        &= \frac{1}{b - a}\int_0^b \left[vc - \frac{c^2}{2}\right]_a^v \, dv + \frac{1}{b - a}\int_b^1 \left[vc - \frac{c^2}{2}\right]_a^b \, dv\\
        &= \frac{1}{2(b - a)}\int_0^b (v - a)^2 \, dv + \frac{1}{b - a}\int_b^1 \left(v(b - a) - \frac{b^2 - a^2}{2}\right) \, dv\\
        &= \frac{1}{2(b - a)}\left[\frac{(v - a)^3}{3}\right]_0^b + \frac{1}{b - a}\left[\frac{(b - a)v^2}{2} - \left(\frac{b^2 - a^2}{2}\right)v\right]_b^1\\
        &= \frac{(b - a)^3 + a^3}{6(b - a)} + \frac{(b - a)(1 - b)(1 - a)}{2(b - a)}\\
        &= \frac{3a^2 - 3a + b^3 - 3b^2 + 3b}{6(b - a)}
        \end{align*}
    \item \begin{align*}
        \frac{1}{b - a}\int_0^1 \int_a^v (v - c) \, dc \, dv
        &= \frac{1}{b - a}\int_0^1 \left[vc - \frac{c^2}{2}\right]_a^v \, dv\\
        &= \frac{1}{b - a}\int_0^1 \left(v(v - a) - \frac{v^2 - a^2}{2}\right) \, dv\\
        &= \frac{1}{2(b - a)}\int_0^1 (v - a)^2 \, dv\\
        &= \frac{1}{2(b - a)}\left[\frac{(v - a)^3}{3}\right]_0^1\\
        &= \frac{3a^2 - 3a + 1}{6(b - a)}
        \end{align*}
    \item \begin{align*}
        \frac{1}{b - a}\int_a^b \int_c^1 (v - c) \, dv \, dc &= \frac{1}{b - a}\int_a^b \left[\frac{v^2}{2} - cv\right]_c^1 \, dc\\
        &= \frac{1}{b - a}\int_a^b \left[\frac{1 - c^2}{2} - c(1 - c)\right] \, dc\\
        &= \frac{1}{2(b - a)}\int_a^b (c - 1)^2\, dc\\
        &= \frac{1}{2(b - a)}\left[\frac{(c - 1)^3}{3}\right]_a^b\\
        &= \frac{(b^3 - a^3) - 3(b^2 - a^2) + 3(b - a)}{6(b - a)}\\
        &= \frac{a^2 + ab + b^2 - 3a - 3b + 3}{6}\\
        \end{align*}
    \item \begin{align*}
        \frac{1}{b - a}\int_a^1 \int_a^v (v - c) \, dc \, dv &= \frac{1}{b - a}\int_a^1 \left[vc - \frac{c^2}{2}\right]_a^v \, dv\\
        &= \frac{1}{b - a}\int_a^1 \left(v(v - a) - \frac{v^2 - a^2}{2}\right) \, dv\\
        &= \frac{1}{2(b - a)}\int_a^1 (v - a)^2 \, dv\\
        &= \frac{1}{2(b - a)}\left[\frac{(v - a)^3}{3}\right]_a^1\\
        &= \frac{(1 - a)^3}{6(b - a)}
        \end{align*}
    \item \begin{align*}
        &\frac{1}{b - a}\int_0^{b + T_a} \int_a^{v - T_a} (v - c) \, dc \, dv + \frac{1}{b - a}\int_{b + T_a}^1 \int_a^b (v - c) \, dc \, dv\\ 
        &= \frac{1}{b - a}\int_0^{b + T_a} \left[vc - \frac{c^2}{2}\right]_a^{v - T_a} \, dv + \frac{1}{b - a}\int_{b + T_a}^1 \left[vc - \frac{c^2}{2}\right]_a^b \, dv\\
        &= \frac{1}{b - a}\int_0^{b + T_a} \left(v(v - T_a - a) - \frac{(v - T_a)^2 - a^2}{2}\right) \, dv + \frac{1}{b - a}\int_{b + T_a}^1 \left[v(b - a) - \frac{b^2 - a^2}{2}\right] \, dv\\ 
        &= \frac{1}{b - a}\int_0^{b + T_a} \left(\frac{v^2}{2} - av - \frac{T_a^2}{2} + \frac{a^2}{2}\right) \, dv + \int_{b + T_a}^1 \left[v - \frac{a + b}{2}\right] \, dv\\ 
        &= \frac{1}{b - a}\int_0^{b + T_a} \left(\frac{v^2}{2} - av + \frac{3a^2 + 2a - 1}{8}\right) \, dv + \int_{b + T_a}^1 \left[v - \frac{a + b}{2}\right] \, dv\\
        &= \frac{1}{b - a}\left[\frac{v^3}{6} - \frac{av^2}{2} + \frac{(3a^2 + 2a - 1)v}{8}\right]_0^{b + T_a} + \left[\frac{v^2}{2} - \frac{(a + b)v}{2}\right]_{b + T_a}^1\\
        &= \frac{(b + T_a)}{b - a}\left(\frac{(b + T_a)^2}{6} - \frac{a(b + T_a)}{2} + \frac{3a^2 + 2a - 1}{8}\right) + \left(\frac{1 - (b + T_a)^2}{2} - \frac{(a + b)(1 - b - T_a)}{2}\right)\\
        &= \frac{(b + T_a)}{b - a}\left(\frac{4b^2 + 8bT_a + 4T_a^2 - 12ab - 12aT_a + 9a^2 + 6a - 3}{24}\right) + \frac{1 - bT_a - T_a^2 - a + ab + aT_a - b}{2}\\
        &= \frac{(b + T_a)}{b - a}\left(\frac{4b^2 + 8bT_a + 4T_a^2 - 12ab - 12aT_a + 9a^2 + 6a - 3}{24}\right) - \frac{(T_a + b - 1)(T_a - a + 1)}{2}\\
        &= \frac{(2b - a + 1)}{2(b - a)}\left(\frac{2b^2 + 2b - 8ab - 1 - a + 8a^2}{12}\right) - \frac{3(a - 2b + 1)(a - 1)}{8}\\
        &= \frac{(2b - a + 1)(2b^2 + 2b - 8ab - 1 - a + 8a^2)}{24(b - a)} - \frac{9(a - 2b + 1)(a - 1)(b - a)}{24(b - a)}\\
        &= \frac{4b^3 + 6b^2 - 18ab^2 - 12ab + 24a^2b + 9a^2 - 8a^3 - 1}{24(b - a)} - \frac{27a^2b - 9a^3 - 18ab - 18ab^2 + 18b^2 - 9b + 9a}{24(b - a)}\\
        &= \frac{4b^3 - 12b^2 + 6ab - 3a^2b + 9a^2 + a^3 - 1 + 9b - 9a}{24(b - a)}\\
        &= \frac{(a + b - 1)(a^2 - 4ab + 10a + 4b^2 - 8b + 1)}{24(a - b)}
        \end{align*}
    \item \begin{align*}
        \frac{1}{b - a}\int_0^1 \int_a^{v - T_a} (v - c) \, dc \, dv &= \frac{1}{b - a}\int_0^1 \left[vc - \frac{c^2}{2}\right]_a^{v - T_a} \, dv\\ 
        &= \frac{1}{b - a}\int_0^1 \left(v(v - T_a - a) - \frac{(v - T_a)^2 - a^2}{2}\right) \, dv\\
        &= \frac{1}{b - a}\int_0^1 \left(\frac{v^2}{2} - av - \frac{T_a^2}{2} + \frac{a^2}{2}\right) \, dv\\
        &= \frac{1}{b - a}\int_0^1 \left(\frac{v^2}{2} - av + \frac{3a^2 + 2a - 1}{8}\right) \, dv\\
        &= \frac{1}{b - a}\left[\frac{v^3}{6} - \frac{av^2}{2} + \frac{(3a^2 + 2a - 1)v}{8}\right]_0^1\\
        &= \frac{1}{b - a}\left(\frac{1}{6} - \frac{a}{2} + \frac{3a^2 + 2a - 1}{8}\right)\\
        &= \frac{(3a - 1)^2}{24(b - a)}
    \end{align*}
    \item \begin{align*}
        \frac{1}{b - a}\int_a^b \int_{c + T_a}^1 (v - c) \, dv \, dc &= \frac{1}{b - a}\int_a^b \left[\frac{v^2}{2} - cv\right]_{c + T_a}^1 \, dc\\ 
        &= \frac{1}{b - a}\int_a^b \left(\frac{1 - (c + T_a)^2}{2} - c(1 - c - T_a)\right) \, dc\\ 
        &= \frac{1}{b - a}\int_a^b \left(\frac{c^2}{2} - c + \frac{1 - T_a^2}{2}\right) \, dc\\
        &= \frac{1}{b - a}\left[\frac{c^3}{6} - \frac{c^2}{2} + \frac{(1 - T_a^2)c}{2}\right]_a^b\\
        &= \frac{1}{b - a}\left(\frac{b^3 - a^3}{6} - \frac{b^2 - a^2}{2} + \frac{(1 - T_a^2)(b - a)}{2}\right)\\
        &= \frac{b^2 + ab + a^2}{6} - \frac{a + b}{2} + \frac{3 + 2a - a^2}{8}\\
        &= \frac{4b^2 + 4ab + 4a^2}{24} - \frac{12a + 12b}{24} + \frac{9 + 6a - 3a^2}{24}\\
        &= \frac{4b^2 + 4ab + a^2 - 6a - 12b + 9}{24}\\
        &= \frac{(a + 2b - 3)^2}{24}
    \end{align*}
    \item \begin{align*}
        \frac{1}{b - a}\int_{a + T_a}^1 \int_a^{v - T_a} (v - c) \, dc \, dv &= \frac{1}{b - a}\int_{a + T_a}^1 \left[vc - \frac{c^2}{2}\right]_a^{v - T_a} \, dv\\
        &= \frac{1}{b - a}\int_{a + T_a}^1 \left(v(v - T_a - a) - \frac{(v - T_a)^2 - a^2}{2}\right) \, dv\\
        &= \frac{1}{b - a}\int_{a + T_a}^1 \left(\frac{v^2}{2} - av - \frac{T_a^2}{2} + \frac{a^2}{2}\right) \, dv\\
        &= \frac{1}{b - a}\int_{a + T_a}^1 \left(\frac{v^2}{2} - av + \frac{3a^2 + 2a - 1}{8}\right) \, dv\\
        &= \frac{1}{b - a}\left[\frac{v^3}{6} - \frac{av^2}{2} + \frac{(3a^2 + 2a - 1)v}{8}\right]_{a + T_a}^1\\
        &= \frac{1}{b - a}\left(\frac{1}{6} - \frac{a}{2} + \frac{3a^2 + 2a - 1}{8}\right)\\ 
        &- \frac{a + T_a}{b - a}\left(\frac{(a + T_a)^2}{6} - \frac{a(a + T_a)}{2} + \frac{3a^2 + 2a - 1}{8}\right)\\
        &= \frac{(3a - 1)^2}{24(b - a)} - \frac{a + T_a}{b - a}\left(\frac{a^2 - 4aT_a + 4T_2^2 + 6a - 3}{24}\right)\\
        &= \frac{(3a - 1)^2}{24(b - a)} - \frac{a + 1}{2(b - a)}\left(\frac{2a^2 + a - 1}{12}\right)\\
        &= \frac{-2a^3 + 6a^2 - 6a + 2}{24(b - a)}\\
        &= \frac{(1 - a)^3}{12(b - a)}\\
        \end{align*}
\end{enumerate}

